An Efficient Framework for Optimistic Concurrent Execution of Smart Contracts

Blockchain platforms such as Ethereum and several others execute complex transactions in blocks through user-defined scripts known as smart contracts. To append a correct block into blockchain, miners execute these transactions of smart contracts sequentially. Later the validators serially re-execute the smart contract transactions of the block to validate it. If validation is successful then the block is added to the blockchain using a consensus protocol and miner gets the incentive. In the current era of multi-core processors, by employing the serial execution of the transactions, the miners and validators fail to utilize the cores properly and as a result, have poor throughput. By entitling concurrency to smart contracts execution, we can achieve better efficiency and higher throughput. In this proposal, we develop a novel and efficient technique to execute the smart contract transactions concurrently by miner using optimistic Software Transactional Memory systems (STMs). The miner proposes a block which consists of the set of transactions, conflict graph, hash of previous block and final state of each shared data-objects. Later, we propose concurrent validator which re-executes the same smart contracts concurrently and deterministically with the help of conflict graph given by miner and verifies the final states. On successful validation, proposed block appended into the blockchain and miner gets the incentive. We consider a benchmarks from solidity documentation. We execute the smart contract transactions concurrently using Basic Time stamp Ordering (BTO) and Multi-Version Time stamp Ordering (MVTO) protocols as optimistic STMs. BTO and MVTO miner achieves 3.6x and 3.7x average speedups over serial miner respectively. BTO and MVTO validator outperform average 40.8x and 47.1x than serial validator respectively.

==> Arxiv version Archit pdp-19-bc (H space) (copy)/Background.tex <==
\section{System Model and Background}
\label{sec:model}
This section includes the commencement of notions related to this paper such as \bc{}, \scontract{s}, STMs and its execution model. Here, we limit our discussion to a well-known smart contracts platform, Ethereum. We improve the throughput by ensuring the concurrent execution of \scontract{s} using an efficient framework, optimistic STMs. 

\subsection{Blockchain and Smart Contracts}
Blockchain is a distributed and highly secure technology which stores the records into the block. It consists of multiple peers (or nodes), and each peer maintains decentralize distributed ledger that makes it publicly readable but tamper-proof. Peer executes some functions in the form of transactions. A transaction is a set of instructions executing in the memory. Bitcoin is a blockchain system which only maintains the balances while transferring the money from one account to another account in the distributed manner. Whereas, the popular blockchain system such as Ethereum maintains the state information as well. Here, transactions execute the atomic code known as a function of \scontract{}. Smart contract consists of one or more atomic-units or functions. In this paper, the atomic-unit contains multiple steps that have been executed by an efficient framework which is optimistic STMs.

\noindent
\textbf{Smart Contracts:} The transactions sent by clients to miners are part of a larger code called as \emph{\scontract{s}} that provide several complex services such as managing the system state, ensures rules, or credentials checking of the parties involved, etc. \cite{Dickerson+:ACSC:PODC:2017}. 
%\Scontract{s} are like a `class' in programming languages that encapsulate data and methods which operate on the data. The data represents the state of the \scontract (as well as the \bc) and the \mth{s} (or functions) are the transactions that possibly can change contract state. A transaction invoked by a client is typically such a \mth or a collection of \mth{s} of a \scontract. The smart contracts are designed in languages which are Turing-complete. Ethereum uses solidity \cite{Solidity} while Hyperledger supports popular language such as Java, Golang, Node.js, etc. 
For better understanding of smart contract, we describe a simple auction contract from Solidity documentation \cite{Solidity}.\\
\textbf{Simple Auction Contract:} The functionality of simple auction contract is shown in \algoref{sa}. Where \Lineref{sa1} declares the contract, followed by public state variables as ``highestBidder, highestBid, and pendingReturn'' which records the state of the contract. A single owner of the contract initiates the auction by executing constructor ``SimpleAuction()'' method (omitted due to lack of space) in which function initialize bidding time as auctionEnd (\Lineref{sa3}). %The constructor is executed during the creation of the contract and cannot be called later. 
There can be any number of participants to bid. The bidders may get their money back whenever the highest bid is raised. For this, a public state variable declared at \Lineref{sa7} (pendingReturns) uses solidity built-in complex data type mapping to maps bidder addresses with unsigned integers (withdraw amount respective to bidder). Mapping can be seen as a hash table with key-value pair. This mapping uniquely identifies account addresses of the clients in the Ethereum blockchain. A bidder withdraws the amount of their earlier bid by calling withdraw() method \cite{Solidity}.

At \Lineref{sa8}, a contract function ``bid()'' is declared, which is called by bidders to bid in the auction. Next, ``auctionEnd'' variable is checked to identify whether the auction already called off or not. Further, bidders ``msg.value'' check to identify the highest bid value at \Lineref{sa11}. Smart contract methods can be aborted at any time via throw when the auction is called off, or bid value is smaller than current ``highestBid''. When execution reaches to \Lineref{sa14}, the ``bid()'' method recovers the current highest bidder data from mapping through the ``highestBidder'' address and updates the current bidder pending return amount. Finally, at \Lineref{sa16} and \Lineref{sa17}, it updates the new highest bidder and highest bid amount.%For better understanding of smart contract, we have considered simple auction contract written in high-level programming language as solidity. It is an auction \SContract{} in which bidders are the shared data-objects. Owner is a person who start the auction after that other participants can start biding. The termination condition for auction is the bidding period (or end time) initializes at the start of the auction. In the bidding period multiple participants can take part in the bid. The participant who bids the highest amount will be successful and transfer the amount from their account to the pending  account. All the \au{s} of the block are requested to bidPlusOne() or withdraw(). Current bidder can request for bidPlusOne() if its amount of bid is higher than previous highest bidder. After that current highest bidder transfers the money back to the previous highest bidder from pending account using withdraw(). Conflict can occur if at least two bidders are going to request for bidPlusOne() simultaneously. Such conflicts can very much transpire when \emph{miner} executes \SContract{s} concurrently. We are handling this conflicts with the help of optimistic STMs and ensuring consistency. Once the bidder period is over the highest bidder amount is transfered from their account to beneficiary account.
%\todo{Explain this algo}

%\vspace{-.3cm}
\begin{algorithm}
	\scriptsize
	\caption{SimpleAuction: It allows every bidder to send their bids throughout the bidding period.}	\label{alg:sa} 
	%\setlength{\multicolsep}{0pt}
	%	\begin{multicols}{2}
	\begin{algorithmic}[1]
		\makeatletter\setcounter{ALG@line}{0}\makeatother
		\Procedure{Contract SimpleAuction}{} \label{lin:sa1}
		%\State contract SimpleAuction \label{lin:sa1}
		\State address public beneficiary;\label{lin:sa2}
		\State uint public auctionEnd;\label{lin:sa3}
		\State /*current state of the auction*/\label{lin:sa4}
		\State address public highestBidder;\label{lin:sa5}
		\State uint public highestBid;\label{lin:sa6}
		\State mapping(address $=>$ uint) pendingReturns; \label{lin:sa7} 
		%		\State // more state definitions
		\Function {}{}bid() public payable \label{lin:sa8}
		
		\If{(now $\geq$ auctionEnd)} %\label{lin:sa9}
		\State throw;\label{lin:sa10}
		\EndIf
		\If{(msg.value $<$ highestBid)} \label{lin:sa11}
		\State thorw;\label{lin:sa12}
		\EndIf
		\If{(highestBid != 0)}\label{lin:sa13}
		\State pendingReturns[highestBidder] += highestBid;\label{lin:sa14}
		\EndIf  \label{lin:sa15}
		\State highestBidder = msg.sender;\label{lin:sa16}
		\State highestBid = msg.value;\label{lin:sa17}
		%		\State emit HighestBidIncreased(msg.sender, msg.value);\label{lin:sa8}
		\EndFunction
		\State // more operation definitions\label{lin:sa18}
		\EndProcedure
		
	\end{algorithmic}
	%	\end{multicols}
\end{algorithm}
% Here, we limit our discussion to a well-known smart contracts platform, Ethereum. %We improve the throughput by ensuring the concurrent execution of \scontract{s} using an efficient framework, optimistic STMs. 

%\subsection{Blockchain and Smart Contracts}
%Blockchain is a distributed and highly secure technology which stores the records into block. It consists of multiple peers (or nodes) and each peer maintains decentralize distributed ledger that makes it publicly readable but tamper-proof. Peers are executing some functions in the form of transactions. Transaction is set of instructions executing in the memory. Bitcoin is a blockchain system which only maintains the balances while transferring the money from one account to another account in distributed manner. Whereas, the popular blockchain system such as Ethereum maintains the state information as well. Here, transactions execute the atomic code known as function of \scontract{}. Smart Contract consists of one or more atomic units or functions. In this paper, The atomic unit contains multiple steps that have been executed by an efficient framework which is optimistic STMs.

\noindent
\textbf{Software Transactional Memory Systems:} Following~\cite{tm-book,KuzSat:NI:TCS:2016}, we assume a system of $n$ processes/threads, $p_1,\ldots,p_n$ that access a collection of \emph{transactional objects} or \tobj{s} via atomic \emph{transactions}. Each transaction has a unique identifier. Within a transaction, processes can perform \emph{transactional operations or \mth{s}}: \textit{\begt{()}} that begins a transaction, \textit{\twrite}$(x,v)$ (or $w(x, v)$) that updates a \tobj{} $x$ with value $v$ in its local memory, \textit{\tread}$(x, v)$ (or $r(x, v)$) that tries to read  $x$ and returns value as $v$, \textit{\tryc}$()$ that tries to commit the transaction and returns $commit$ (or $\commit$) if it succeeds, and \textit{\trya}$()$ that aborts the transaction and returns $\abort$. %For the sake of presentation simplicity, we assume that the values taken as arguments by \textit{\twrite{()}} operations are unique. 
Operations \textit{\tread{()}} and \textit{\tryc}$()$ may return $\abort{}$. %, in which case we say that the operations \emph{forcefully abort}. Otherwise, we say that the operations have \emph{successfully} executed.  Each operation is equipped with a unique transaction identifier. 
Transaction $T_i$ starts with the first operation and completes when any of its operations return $\abort$ or $\commit$. %We denote any \op{} that returns $\abort$ or $\commit$ as \emph{\termop{s}}. Hence, \op{s} \textit{\tryc{()}} and \textit{\trya{()}} are \emph{\termop{s}}. A transaction does not invoke any further \op{s} after \emph{\termop{s}}.
For a transaction $T_k$, we denote all the \tobj{s} accessed by its read \op{s} and write operations as $\rs_k$ and $\ws_k$ respectively.  We denote all the \op{s} of a transaction $T_k$ as $\evts{T_k}$ or $evts_k$. 

\noindent
\textbf{History:}
A \emph{history} is a sequence of \emph{events}, i.e., a sequence of 
invocations and responses of transactional operations. The collection of events 
is denoted as $\evts{H}$. For simplicity, we only consider \emph{sequential} 
histories here: the invocation of each transactional operation is immediately followed by a matching response. Therefore, we treat each transactional operation as one atomic event and let $<_H$ denote the total order on the 
transactional operations incurred by $H$. %With this assumption, the only relevant events of a transaction $T_k$ is of the types: $r_k(x,v)$, $r_k(x,\abort)$, $w_k(x, v)$, $\tryc_k(\commit)$ (or $c_k$ for short), $\tryc_k(\abort)$, $\trya_k(\abort)$ (or $a_k$ for short).  
We identify a 
history $H$ as tuple $\langle \evts{H},<_H \rangle$. 

%Let $H|T$ denote the history consisting of events of $T$ in $H$, and $H|p_i$ denote the history consisting of events of $p_i$ in $H$. 
We only consider \emph{well-formed} histories here, i.e., no transaction of a process begins before the previous transaction invocation has completed (either $commits$ or $aborts$). We also assume that every history has an initial \emph{committed} transaction $T_0$ that initializes all the t-objects with value $0$. The set of transactions that appear in $H$ is denoted by $\txns{H}$. The set of \emph{committed} (resp., \emph{aborted}) transactions in $H$ is denoted by $\comm{H}$ (resp., $\aborted{H}$). The set of \emph{incomplete} or \emph{live} transactions in $H$ is denoted by $\incomp{H} = \live{H} = (\txns{H}-\comm{H}-\aborted{H})$. 

We construct a \emph{complete history} of $H$, denoted as $\overline{H}$, by inserting $\trya_k(\abort)$ immediately after the last event of every transaction $T_k\in \live{H}$. But for $\tryc_i$ of transaction $T_i$, if it released the lock on first \tobj{} successfully that means updates made by $T_i$ is consistent so, $T_i$ will immediately return commit.
\cmnt{
\noindent
\textbf{Sub-history:} A \textit{sub-history} ($SH$) of a history ($H$) 
denoted as the tuple $\langle \evts{SH},$ $<_{SH}\rangle$ and is defined as: 
(1) $<_{SH} \subseteq <_{H}$; (2) $\evts{SH} \subseteq \evts{H}$; (3) If an 
event of a transaction $T_k\in\txns{H}$ is in $SH$ then all the events of $T_k$ 
in $H$ should also be in $SH$. 

For a history $H$, let $R$ be a subset of $\txns{H}$. Then $\shist{R}{H}$ denotes  the \ssch{} of $H$ that is formed  from the \op{s} in $R$.
}

\noindent
%\textbf{Transaction orders:} For two transactions $T_k,T_m \in 
\textbf{\textit{Transaction Real-Time and Conflict order:}} For two transactions $T_k,T_m \in \txns{H}$, we say that  $T_k$ \emph{precedes} $T_m$ in the \emph{real-time order} of $H$, denoted as $T_k\prec_H^{RT} T_m$, if $T_k$ is complete in $H$ and the last event of $T_k$ precedes the first event of $T_m$ in $H$. If neither $T_k \prec_H^{RT} T_m$ nor $T_m \prec_H^{RT} T_k$, then $T_k$ and $T_m$ \emph{overlap} in $H$. We say that a history is \emph{\tseq} if all the transactions are ordered by real-time order. %Note that from our earlier assumption all the transactions of a single process are ordered by real-time.

%\ignore{
We say that $T_k, T_m$ are in conflict, denoted as $T_k\prec_H^{Conf} T_m$, if (1) $\tryc_k()<_H \tryc_m()$ and $wset(T_k) \cap wset(T_m) \neq\emptyset$; (2) $\tryc_k()<_H r_m(x,v)$, $x \in wset(T_k)$ and $v \neq \abort$; (3) $r_k(x,v)<_H \tryc_m()$, $x\in wset(T_m)$ and $v \neq \abort$. Thus, it can be seen that the conflict order is defined only on \op{s} that have successfully executed. We denote the corresponding \op{s} as conflicting. 
%}

\noindent
\textbf{Valid and Legal histories:} A successful read $r_k(x, v)$ (i.e., $v \neq \abort$)  in a history $H$ is said to be \emph{\valid} if there exist a transaction $T_j$ that wrote $v$ to $x$ and \emph{committed} before $r_k(x,v)$. %Formally, $\langle r_k(x, v)$  is \valid{} $\Leftrightarrow \exists T_j: (c_j <_{H} r_k(x, v)) \land (w_j(x, v) \in \evts{T_j}) \land (v \neq \abort) \rangle$.  
History $H$ is \valid{} if all its successful read \op{s} are \valid. 

We define $r_k(x, v)$'s \textit{\lastw{}} as the latest commit event $\commit_i$ preceding $r_k(x, v)$ in $H$ such that $x\in wset_i$ ($T_i$ can also be $T_0$). A successful read \op{} $r_k(x, v)$ (i.e., $v \neq \abort$), is said to be \emph{\legal{}}  if the transaction containing $r_k$'s \lastw{} also writes $v$ onto $x$.%:  $\langle r_k(x, v)$ \text{is \legal{}} $\Leftrightarrow (v \neq \abort) \land (\lwrite{r_k(x, v)}{H} = c_i) \land (w_i(x,v) \in \evts{T_i})\rangle$.  
 The history $H$ is \legal{} if all its successful read \op{s} are \legal.  From the definitions we get that if $H$ is \legal{} then it is also \valid.

%
%Let $H$ be a history and $r_k(x, v)$ be a read {\op} in $H$. 

\noindent
\textbf{Notions of Equivalence:} Two histories $H$ and $H'$ are \emph{equivalent} if they have the same set of events. We say two histories $H, H'$ are \emph{multi-version view equivalent} \cite[Chap. 5]{WeiVoss:TIS:2002:Morg} or \emph{\mvve} if (1) $H, H'$ are valid histories and (2) $H$ is equivalent to $H'$. 

Two histories $H, H'$ are \emph{view equivalent} \cite[Chap. 3]{WeiVoss:TIS:2002:Morg} or \emph{\vie} if (1) $H, H'$ are legal histories and (2) $H$ is equivalent to $H'$. By restricting to \legal{} histories, view equivalence does not use multi-versions. 

Two histories $H, H'$ are \emph{conflict equivalent} \cite[Chap. 3]{WeiVoss:TIS:2002:Morg} or \emph{\ce} if (1) $H, H'$ are legal histories and (2) conflict in $H, H'$ are the same, i.e., $conf(H) = conf(H')$. Conflict equivalence like view equivalence does not use multi-versions and restricts itself to \legal{} histories. 
%\todo{Define conf(H) in similar to RT order. DONE}
%, View-Equivalence and Multi-Version View-Equivalence

\noindent
\textbf{VSR, MVSR, and CSR:} A history $H$ is said to VSR (or View Serializable) \cite[Chap. 3]{WeiVoss:TIS:2002:Morg}, if there exist a serial history $S$ such that $S$ is view equivalent to $H$. But it maintains only one version corresponding to each \tobj{}.

So, MVSR (or Multi-Version View Serializable) came into picture which maintains multiple version corresponding to each \tobj. A history $H$ is said to MVSR \cite[Chap. 5]{WeiVoss:TIS:2002:Morg}, if there exist a serial history $S$ such that $S$ is multi-version view equivalent to $H$. It can be proved that verifying the membership of VSR as well as MVSR in databases is NP-Complete \cite{Papad:1979:JACM}. To circumvent this issue, researchers in databases have identified an efficient sub-class of VSR, called CSR based
on the notion of conflicts. The membership of CSR can be verified in polynomial time using conflict graph characterization. 

A history $H$ is said to CSR (or Conflict Serializable) \cite[Chap. 3]{WeiVoss:TIS:2002:Morg}, if there exist a serial history $S$ such that $S$ is conflict equivalent to $H$.
\\
\noindent
\textbf{Serializability and Opacity:} 
Serializability\cite{Papad:1979:JACM} is a commonly used criterion in databases. But it is not suitable for STMs as it does not consider the correctness of \emph{aborted} transactions as shown by Guerraoui \& Kapalka \cite{GuerKap:Opacity:PPoPP:2008}. Opacity, on the other hand, considers the correctness of \emph{aborted} transactions as well.

A history $H$ is said to be \textit{opaque} \cite{GuerKap:Opacity:PPoPP:2008,tm-book} if it is \valid{} and there exists a t-sequential legal history $S$ such that (1) $S$ is equivalent to complete history $\overline{H}$ and (2) $S$ respects $\prec_{H}^{RT}$, i.e., $\prec_{H}^{RT} \subset \prec_{S}^{RT}$.  By requiring $S$ being equivalent to $\overline{H}$, opacity treats all the incomplete transactions as aborted. %We  call $S$ an (opaque) \emph{serialization} of $H$.

\cmnt{
Along same lines, a \valid{} history $H$ is said to be \textit{strictly serializable} if $\shist{\comm{H}}{H}$ is opaque. Unlike opacity, strict serializability does not include aborted or incomplete transactions in the global serialization order. An opaque history $H$ is also strictly serializable: a serialization of $\shist{\comm{H}}{H}$ is simply the subsequence of a serialization of $H$ that only contains transactions in $\comm{H}$. 
}



%\todo{Define VSR, MVSR, CSR in terms of equivalence. Then define opacity along the same lines. DONE}
\cmnt{
\noindent 
\textbf{VSR, MVSR, and CSR:} VSR (or View Serializability) is a correctness-criterion same as opacity but it does not consider aborted transactions. When the protocol (such as MVTO) maintains multiple versions corresponding to each \tobj{} then a commonly used correctness criterion in databases is MVSR (or Multi-Version View Serializability). It can be proved that verifying the membership of VSR as well as MVSR in databases is NP-Complete \cite{Papad:1979:JACM}. To circumvent this issue, researchers in databases have identified an efficient sub-class of VSR, called CSR (or conflict-serializability), based
on the notion of conflicts. The membership of CSR can be verified in polynomial time using conflict graph characterization. 
}

\noindent
\textbf{Linearizability:} A history $H$ is linearizable \cite{HerlihyandWing:1990:LCC:ACM} if (1) The invocation and response events can be reordered to get a valid sequential history.
(2) The generated sequential history satisfies the object’s sequential specification. (3) If a response event precedes an invocation event in the original history, then this should be preserved in the sequential reordering.

\noindent
\textbf{Lock Freedom:} An algorithm is said to be lock-free\cite{HerlihyShavit:Progress:Opodis:2011} if the program threads are run for a sufficiently long time, at least one of the threads makes progress. It allows individual threads to starve but guarantees system-wide throughput.

\ignore{

%\subsection{Blockchain}

\begin{enumerate}
	\item BTO 
	\begin{itemize}
		\item Conflicts.
	\end{itemize}
	\item MVTO 
	\begin{itemize}
		\item Conflicts.
	\end{itemize}
\end{enumerate}
}

==> Arxiv version Archit pdp-19-bc (H space) (copy)/conclusion.tex <==
\vspace{-.3cm}
\section{Conclusion}
\label{sec:con}
To exploit the multi-core processors, we have proposed the concurrent execution of \scontract{} by miners and validators which improves the throughput. Initially, miner executes the smart contracts concurrently using optimistic STM protocol as BTO. To reduce the number of aborts and improves the efficiency further, the concurrent miner uses MVTO protocol which maintains multiple versions corresponding to each data-object. %After that it forms a BG concurrently, which ensures non-conflicting transactions can run parallelly. 
Concurrent miner proposes a block which consists of a set of transactions, BG, hash of the previous block and final state of each shared data-objects. Later, the validators re-execute the same \SContract{} transactions concurrently and deterministically with the help of BG given by miner which capture the conflicting relations among the transactions to verify final state. If the validation is successful then proposed block appended into the blockchain and miner gets incentive otherwise discard the proposed block. Overall, BTO and MVTO miner performs
3.6x and 3.7x speedups over serial miner respectively. Along with, BTO and MVTO validator outperform average 40.8x and 47.1x than serial validator respectively. 

\vspace{1mm}
\noindent
\textbf{Acknowledgements.} This project is in part supported by a research grant from Thynkblynk Technologies Pvt. Ltd, and IMPRINT India scheme. We are grateful to Dr. Bapi Chatterjee, Dr. Sandeep Hans, Mr. Ajay Singh for several useful discussions that we had on this topic. We would like to thank anonymous reviewers for their useful comments. We are also very grateful to Anila Kumari  and G Monika the developers of IITH STM. 

==> Arxiv version Archit pdp-19-bc (H space) (copy)/correctness.tex <==
\section{Correctness}
\label{sec:correctness}

\subsection{The Linearization Points of Lock-free Graph Library Methods}

Here, we list the linearization points (LPs) of each method as follows:

\begin{enumerate}
	\item \addv{(\vgn)}: (\vp.\vn.CAS(\vc, \vgn)) in \Lineref{addv5} is the LP point of \addv{()} method if \vnode{} is not exist in the BG. If \vnode{} is exist in the BG then (\vc.$ts_i$ $\neq$ \vgn.$ts_i$) in \Lineref{addv3} is the LP point.
	
	\item \adde{\emph{(fromNode, toNode)}}: 		(\ep.\en.CAS(\ec, \egn)) in \Lineref{adde7} is the LP point of \adde{()} method if \enode{} is not exist in the BG. If \enode{} is exist in the BG then 		(\ec.$ts_i$ $\neq$ toNode.$ts_i$) in \Lineref{adde5} is the LP point.
	
	\item \searchl{(cacheVer, $AU_{id}$)}: (cacheVer.\inc.CAS(0, -1)) in \Lineref{sl1} is the LP point of \searchl{()} method.
	
	\item \searchg{(BG, $AU_{id}$)}: (\vnode.\inc.CAS(0, -1)) in \Lineref{sg1} is the LP point of \searchg{()} method.
	
	\item \emph{decInCount}(remNode): \Lineref{ren1} is the LP point of \emph{decInCount()} method.
\end{enumerate}


\begin{theorem}
	All the dependencies between the conflicting nodes are captured in the BG.
\end{theorem} 

\begin{proof}
	Dependencies between the conflicting nodes are captured in the BG with the help of LP points of lock-free graph library methods defined above.
\end{proof}


\cmnt{

\begin{lemma}
History $H_m$ generated by BTO protocol and $H_v$ are view equivalent.
\end{lemma}



Concurrent execution of \SContract{s} may lead to inconsistent state, if it is not done carefully. In the concurrent execution of \miner, multiple threads are running concurrently and they can run in any order. But, if we achieve any equivalent serial execution of the concurrent execution then we can ensure that execution done by \conminer{} is consistent. 

So, we use an efficient framework, \emph{Software Transactional Memory system (STMs)} for the concurrent execution of \SContract{s} in optimistic manner by \miner. STMs are popular programming paradigm which take care of synchronization issues among the transactions and ensure atomicity. Being a programmer who is using the STM library, need not have to worry about consistency issues because STM library ensures the consistency of concurrent execution which is equivalent to some serial execution. We have started with one of the fashionable protocol of STMs as \emph{Basic Timestamp Ordering (STM\_BTO)} which executes non-conflicting transactions concurrently.
\begin{lemma}
	Any concurrent execution of transactions generated by STM\_BTO protocol produces conflict serializable schedule. \cite{WeiVoss:TIS:2002:Morg}
\end{lemma}
If two transactions $T_i$ and $T_j$ are accessing any common shared \tobj{} say $x$ and $ts_i$ is less than $ts_j$  but $T_j$ committed before $T_i$ then STM\_BTO protocol aborts the $T_i$ and retry it again. STM\_BTO protocol produces conflict serializable schedule which follows increasing order of transactions timestamp. It ensures deadlock-freedom by accessing the shared \tobj{s} in increasing order. 

Now, how can we ensure that the execution order done by \conminer{} are same as execution done by \convalidator{s}? To ensure not to reject the correct block by \convalidator{s}, we have used the concept of \cgraph{}. While executing the \SContract{s} by \conminer{} using optimistic STMs, it also maintains all the relevant conflicts in \cgraph{} concurrently. \Cgraph{} captures the dependency among the conflicting transactions and says what all transactions can run concurrently. Finally, \conminer{} proposes a block which consist of set of transactions, \cgraph, hash of previous block and final state of each shared \tobj{s} and send it to the \convalidator{s} to validate it. Later, the \convalidator{s} re-execute the same \SContract{} concurrently and deterministically with the help of \cgraph{} given by \conminer{} and verify the final state. If the final state matches then proposed block appended into the blockchain and miner gets incentive otherwise discard the proposed block.


To improve the concurrency further, we use an another prominent STM protocol as \emph{Multi-Version Timestamp Ordering (STM\_MVTO)}. It also follow the increasing order of timestamp to generate the multi-version conflict serializable schedule and ensure the deadlock-freedom same as STM\_BTO. 
\begin{lemma}
	Any concurrent execution of transactions generated by STM\_MVTO protocol produces multi-version conflict serializable schedule. \cite{Kumar+:MVTO:ICDCN:2014}
\end{lemma}

\cmnt{
\section{Requirements of the Concurrent Miner and Validator}
\label{sec:reqminerval}
The section describes the requirements of concurrent Miner and validator.
\begin{theorem}
Any history $H_m$ generated Concurrent miner should satisfy opacity.
\end{theorem}

Here, miner executes the smart contract concurrently with the help of optimistic STM protocols (BTO and MVTO). Internally, BTO and MVTO \cite{Kumar+:MVTO:ICDCN:2014} protocol ensures opacity. So, history $H_m$ generated Concurrent miner satisfies opacity.

Consider the history $H_m$ generated by BTO protocol and constructs block graph, $BG$ in which each committed transaction $T_i$ consider as vertices and edges between them as follows:
\begin{itemize}
\item r-w: After $T_i$ reads $x$ from $T_k$, $T_j$ writes on $x$ data-object then r-w edge will be from $T_i$ to $T_j$.  
\item w-r: If $T_i$ reads $x$ from the value written by $T_j$ then w-r edge will be from $T_i$ to $T_j$. 
\item w-w:
\end{itemize}
Concrrent miner provides $BG$ to concurrent validators to ensure the correct output by validators. After that concurrent validator apply topological sort on $BG$ and generates a history $H_v$.
\begin{lemma}
History $H_m$ generated by BTO protocol and $H_v$ are view equivalent.
\end{lemma}

\begin{theorem}
History $H_m$ generated by MVTO protocol and $H_v$ are multi-version view equivalent.
\end{theorem}
}

\subsection{The Linearization Points of Lock-free Graph Library Methods}

Here, we list the linearization points (LPs) of each method. Note that each method can return either true or false. So,
we define the LP for five methods:

\begin{enumerate}
\item addVertex()
\end{enumerate}

}





==> Arxiv version Archit pdp-19-bc (H space) (copy)/intro.tex <==
\section{Introduction}
\label{sec:intro}
It is commonly believed that \bc{} is a revolutionary technology for doing business over the Internet. \BC is a decentralized, distributed database or ledger of records. Cryptocurrencies such as Bitcoin \cite{Nakamoto:Bitcoin:2009} and Ethereum \cite{ethereum} were the first to popularize the \bc technology. \BC{s} ensure that the records are tamper-proof but publicly readable. 

Basically, the \bc network consists of multiple peers (or nodes) where the peers do not necessarily trust each other. Each node maintains a copy of the distributed ledger. \emph{Clients}, users of the \bc, send requests or \emph{transactions} to the nodes of the \bc called as \emph{miners}. The miners collect multiple transactions from the clients and form a \emph{block}. Miners then propose these blocks to be added to the \bc. 
%Multiple miners propose new blocks to be added to the distributed ledger. 
They follow a global consensus protocol to agree on which blocks are chosen to be added and in what order. While adding a block to the \bc, the miner incorporates the hash of the previous block into the current block. This makes it difficult to tamper with the distributed ledger. The resulting structure is in the form of a linked list or a chain of blocks and hence the name \bc. 

The transactions sent by clients to miners are part of a larger code called as \emph{\scontract{s}} that provide several complex services such as managing the system state, ensuring rules, or credentials checking of the parties involved \cite{Dickerson+:ACSC:PODC:2017}. \Scontract{s} are like a `class' in programming languages that encapsulate data and methods which operate on the data. The data represents the state of the \scontract (as well as the \bc) and the \mth{s} (or functions) are the transactions that possibly can change contract state. A transaction invoked by a client is typically such a \mth or a collection of \mth{s} of the \scontract{s}. Ethereum uses Solidity \cite{Solidity} while Hyperledger supports language such as Java, Golang, Node.js etc. 

\vspace{1mm}
\noindent
\textbf{Motivation for Concurrent Execution of Smart Contracts: }
As observed by Dickerson et al. \cite{Dickerson+:ACSC:PODC:2017}, \scontract transactions are executed in two different contexts specifically in Ethereum. First, they are executed by miners while forming a block. A miner selects a sequence of client request transactions, executes the smart contract code of these transactions in sequence, transforming the state of the associated contract in this process. The miner then stores the sequence of transactions, the resulting final state of the contracts in the block along with the hash of the previous block. After creating the block, the miner proposes it to be added to the \bc through the consensus protocol.

Once a block is added, the other peers in the system, referred to as \emph{validators} in this context, validate the contents of the block. They re-execute the \scontract transactions in the block to verify the block's final states match or not. If final states match, then the block is accepted as valid and the miner who appended this block is rewarded. Otherwise, the block is discarded. Thus the transactions are executed by every peer in the system. In this setting, it turns out that the validation code runs several times more than miner code \cite{Dickerson+:ACSC:PODC:2017}. 
%it turns out that a block's transactions are validated several more times than when created by the miner \cite{Dickerson+:ACSC:PODC:2017}. %The validators execute the transaction (associated contract code) to check the state of the blockchain. 

This design of \scontract execution is not very efficient as it does not allow any concurrency. Both the miner and the validator execute transactions serially one after another. In today's world of multi-core systems, the serial execution does not utilize all the cores and hence results in lower throughput. This limitation is not specific only to Ethereum but almost all the popular \bc{s}. Higher throughput means more number of transactions executed per unit time by miners and validators which clearly will be desired by both of them.  

\ignore{
\figref{sece} illustrates the motivation behind the execution of smart contracts by concurrent miner over serial miner. Consider \figref{sece} (a) which consists of two transactions $T_1$, and $T_2$ executed by the serial miner. Here, $T_1$, and $T_2$ are writing on data-objects $x$, and $y$ respectively. Due to the  serial execution by miner, all the transactions are executing serially although they are working on different data-objects which tends to limit the throughput of miner. Whereas \figref{sece} (b) represents the concurrent execution by miner with same scenario as \figref{sece} (a) where $T_1$ and $T_2$ are running concurrently because they are working on different data-objects. Hence, concurrent execution by miner improves the throughput as compare to serial miner.
\begin{figure}
	%	\captionsetup{justification=centering}
	\centerline{\scalebox{0.35}{\input{figs/sece.pdf_t}}}
	\caption{Efficient execution of smart contracts}
	\label{fig:sece}
\end{figure}
}

But the concurrent execution of \scontract transactions is not an easy task. The various transactions requested by the clients could consist of conflicting access to the shared data-objects. Arbitrary execution of these transactions by the miners might result in the data-races leading to the inconsistent final state of the \bc. Unfortunately, it is not possible to statically identify if two contract transactions are conflicting or not since they are developed in Turing-complete languages. The common solution for correct execution of concurrent transactions is to ensure that the execution is \emph{\sble} \cite{Papad:1979:JACM}. A usual \cc in databases, \sbty ensure that the concurrent execution is equivalent to some serial execution of the same transactions. Thus the miners must ensure that their execution is \sble \cite{Dickerson+:ACSC:PODC:2017} or one of its variants as described later.
% these have to be executed carefully. Otherwise, it %Hence, miners have to carefully execute these transaction concurrently. 

The concurrent execution of the \scontract transactions of a block by the validators although highly desirable can further complicate the situation. Suppose a miner ensures that the concurrent execution of the transactions in a block are \sble. Later a validator executes the same transactions concurrently. But during the concurrent execution, the validator may execute two conflicting transactions in an order different from what was executed by the miner. Thus the serialization order of the miner is different from the validator. Then this can result in the validator obtaining a final state different from what was obtained by the miner. Consequently, the validator may incorrectly reject the block although it is valid. \figref{conmv} illustrates this in the following example. \figref{conmv} (a) consists of two concurrent conflicting transactions $T_1$ and $T_2$ working on same shared data-objects $x$ which are part of a block. \figref{conmv} (b) represents the concurrent execution by miner with an equivalent serial schedule as $T_1$, $T_2$ and final state (or FS) as 20 from the initial state (or IS) 0. Whereas \figref{conmv} (c), shows the concurrent execution by a validator with an equivalent serial schedule as $T_2$, $T_1$, and final state as 10 from IS 0 which is different from the final state proposed by the miner. Such a situation leads to rejection of the valid block by the validator which is undesirable.
\vspace{-.5cm}
\begin{figure}[H]
%\captionsetup{justification=centering}
	\centerline{\scalebox{0.29}{\input{figs/conMV.pdf_t}}}
\vspace{-.3cm} 	\caption{Execution of concurrent transactions by miner and validator}
	\label{fig:conmv}
\end{figure}
\vspace{-.4cm}
These important issues were identified by Dickerson et al. \cite{Dickerson+:ACSC:PODC:2017} who proposed a solution of concurrent execution for both the miners and validators. In their solution, the miners concurrently execute the transactions of a block using abstract locks and inverse logs to generate a serializable execution. Then, to enable correct concurrent execution by the validators, the miners also provide a \emph{\hb} graph in the block. The \hb graph is a direct acyclic graph over all the transaction of the block. If there is a path from a transaction $T_i$ to $T_j$ then the validator has to execute $T_i$ before $T_j$. Transactions with no path between them can execute concurrently. The validator using the \hb graph in the block executes all the transactions concurrently using the fork-join approach. This methodology ensures that the final state of the \bc generated by the miners and the validators are the same for a valid block and hence not rejected by the validators. The presence of tools such as a \hb graph in the block provides greater enhancement to validators to consider such blocks as it helps them execute quickly by means of parallelization as opposed to a block which does not have any tools for parallelization. This, in turn, entices the miners to provide such tools in the block for concurrent execution by the validators. 

%is indeed labeled as valid by a validator while concurrently executing the trans\hbactions. 

\ignore {

\figref{cminer}, illustrates the functionality of concurrent miner which consists of six steps. It has two or more serial miner and one concurrent miner competing to each other to propose a block in blockchain. Whoever will propose a block first that miner have a chance to get strong incentive. So the challenge here is to execute the task of miner concurrently. All the miners are getting the set of transactions from distributed shared memory. As we discussed above, serial miner executes the transactions one after another and propose the block. Where as concurrent miner executes the non-conflicting transactions concurrently with the help of Transactional Memory (TM) and finally propose a block. Complete details about the \figref{cminer} presents in the \subsecref{cminer}.

\begin{figure}
	\centering
	\captionsetup{justification=centering}
	\centerline{\scalebox{0.45}{\input{figs/cminer.pdf_t}}}
	\caption{Execution of Concurrent Miner}
	\label{fig:cminer}
\end{figure}

}

\vspace{1mm}
\noindent
\textbf{Our Solution Approach - Optimistic Concurrent Execution and Lock-Free Graph: } Dickerson et al. \cite{Dickerson+:ACSC:PODC:2017} developed a solution to the problem of concurrent miner and validators using locks and inverse logs. It is well known that locks are pessimistic in nature. So, in this paper, we explore a novel and efficient framework for concurrent miners using optimistic Software Transactional Memory Systems (STMs).

The requirement of the miner, as explained above, is to concurrently execute the \scontract transactions correctly and output a graph capturing dependencies among the transactions of the block such as \hb graph. We denote this graph as \emph{\bg} (or BG). In the proposed solution, the miner uses the services of an optimistic STM system to concurrently execute the \scontract transactions. Since STMs also work with transactions, we differentiate between \scontract transactions and STM transactions. The STM transactions invoked by an STM system is a piece of code that it tries to execute atomically even in presence of other concurrent STM transactions. If the STM system is not able to execute it atomically, then the STM transaction is aborted. 

The expectation of a \scontract transaction is that it will be executed serially. Thus, when it is executed in a concurrent setting, it is expected to be executed atomically (or serialized). But unlike STM transaction, a \scontract transaction cannot be committed or aborted. Thus to differentiate between \scontract transaction from STM transaction, we denote \scontract transaction as \emph{Atomic Unit} or \emph{\au} and STM transaction as transaction in the rest of the document. Thus the miner uses the STM system to invoke a transaction for each \au. In case the transaction gets aborted, then the STM repeatedly invokes new transactions for the same \au until a transaction invocation eventually commits. 

A popular correctness guarantee provided by STM systems is \emph{\opty} \cite{GuerKap:Opacity:PPoPP:2008} which is stronger than \sbty. Opacity like \sbty requires that the concurrent execution including the aborted transactions be equivalent to some serial execution. This ensures that even aborted transaction reads consistent value until the point of abort. As a result, that the application such as a miner using an STM does not encounter any undesirable side-effects such as crash failures, infinite loops, divide by zero etc. STMs provide this guarantee by executing optimistically and support atomic (\opq) reads, writes on \emph{transactional objects} or \emph{\tobj{s}}. 

Among the various STMs available, we have chosen two timestamp based STMs in our design: (1) \emph{Basic Timestamp Ordering} or \emph{BTO} STM \cite[Chap 4]{WeiVoss:TIS:2002:Morg}, maintains only one version for each \tobj. (2) \emph{Multi-Version Timestamp Ordering} or \emph{\mvto} STM \cite{Kumar+:MVTO:ICDCN:2014}, maintains multiple versions corresponding to each \tobj{} which further reduces the number of aborts and improves the throughput. 

The advantage of using timestamp based STM is that in these systems the equivalent serial history is ordered based on the timestamps of the transactions. Thus using the timestamps, the miner can generate the BG of the \au{s}. Dickerson et al. \cite{Dickerson+:ACSC:PODC:2017}, developed the BG in a serial manner. In our approach, the graph is developed by the miner in concurrent and lock-free \cite{HerlihyShavit:Progress:Opodis:2011} manner. 

%The validator process re-executes all the \au{s}. 
The validator process creates multiple threads. Each of these threads parses the BG and re-execute the atomic-units for validation. The BG provided by concurrent miner shows dependency among the \au{s}. Each validator thread, claims a node which does not have any dependency, i.e. a node without any incoming edges by marking it. After that, it executes the corresponding \au{s} deterministically. Since the threads execute only those nodes that do not have any incoming edges, the concurrently executing \au{s} will not have any conflicts. Hence the validator threads need not have to worry about synchronization issues. We denote this approach adopted by the validator as a decentralized approach (or Decentralized Validator) as the multiple threads are working on BG concurrently in the absence of master thread. 

The approach adopted by Dickerson et al. \cite{Dickerson+:ACSC:PODC:2017}, works on fork-join in which a master thread allocates different tasks to slave threads. The master thread will identify those \au{s} which do not have any dependencies from the BG and allocates them to different slave threads to work on. In this paper, we compare the performance of both these approaches with the serial validator. 

%unlike the fork-join approach adopted by Dickerson et al. \cite{Dickerson+:ACSC:PODC:2017}%

\ignore{
executing \au does not have any conflicts, it 
At any time, the validator executes only those \au{s} concurrently which don't have any dependency as shown by the block graph. We consider the concurrent execution by validator in two different manners. The first one is inspired by Dickerson et al. \cite{Dickerson+:ACSC:PODC:2017} called as fork-join validator. The proposed fork-join validator works on master-slave concept in which a master or central thread allocates the task to slave threads. We propose a concurrent validator using decentralized approach (or Decentralized Validator) in which multiple threads are working on block graph concurrently and deterministically in the absence of master thread. 

In order to execute \scontract{} by concurrent miner, we start with the well known protocol of STMs which is Basic Timestamp Ordering (or STM\_BTO) protocol. STM\_BTO identifies the conflicts between two transactions at run-time and abort one of them and retry again for aborted transaction. It ensures serial order of concurrent execution of transactions which is equivalent to the increasing order of transaction's timestamp. It has been observed by Kumar et al., \cite{Kumar+:MVTO:ICDCN:2014} that storing multiple versions, more concurrency can be gained. So, we motivated towards another popular protocol of STMs which is Multi-Version Timestamp Ordering (or STM\_MVTO) protocol. It store multiple versions corresponding to each data-object so, STM\_MVTO reduces the number of aborts and improves the throughput. STM\_MVTO protocol is also ensuring equivalent serial order as STM\_BTO.

Now, we propose the concurrent validator which is re-executing the same \SContract{} that has been executed by concurrent miner. But it may construct different serial order and different final state than serial order and final state produced by concurrent miner. That may lead to reject the correct proposed block. In order to solve this issue, concurrent miner maintains conflict graph in the form of adjacency-list. Once the transaction commit it adds itself as a vertex into the conflict graph, which is having an edge belonging to each conflicting transactions. %But the main challenge with STM\_MVTO protocol is to maintain the correct conflict-list, which is required to maintain the conflict graph in the form of adjacency-list. It maintains the conflict in the form of adjacency-list and reduces the size of conflict-list so, improves the performance.

So, concurrent validator executes the transactions deterministically and concurrently with the help of conflict graph given by the miner. It applies the topological sort on the graph and identify the vertex whose indegree is 0. It then execute the \SContract{} concurrently corresponding to identified vertex and compute the final state. %Once the execution over it removes the outgoing edges from the conflict graph and decrease the in-count of conflicting vertices. Concurrently all the threads are finding the source node with indegree 0 till the CG will have no source node. 
Eventually, it compare the final state present in the block proposed by the miner with its computed final state corresponding to each data-object. If its same then block is appended into the blockchain and concurrent miner rewarded with strong incentive. Otherwise, block is discarded.
}

\noindent
\textbf{Contributions of the paper as follows:}
\begin{itemize}
%\item % What is \bc?
%\item What is \scontract?
%\item Why we need to add the concurrency in \scontract?
%\item How STMs going to help to add concurrency in \scontract?
\item Introduce a novel way to execute the \SContract{} transactions by concurrent miner using optimistic STMs.% that allows non-conflicting transactions to execute concurrently.
\item We implement the concurrent miner with the help of BTO and MVTO STM but its generic to any STM protocol.

\item We propose a lock-free graph library to generate the BG.
\item We propose concurrent validator that re-executes the \SContract{} transactions deterministically and efficiently with the help of BG given by concurrent miner.

\item Concurrent miner satisfies correctness criterion as opacity. 
\item We achieve 3.6x and 3.7x average speedups for concurrent miner using BTO and MVTO STM protocol respectively. Along with, BTO and MVTO validator outperform average 40.8x and 47.1x than serial validator respectively.  

%BTO and MVTO miner performs
%3.2 and 3.3 speedups over serial miner respectively. 
\end{itemize}

\noindent
\textbf{Related Work:} The first \emph{blockchain} concept has been given by Satoshi Nakamoto in 2009 \cite{Nakamoto:Bitcoin:2009}. He proposed a system as bitcoin \cite{Nakamoto:Bitcoin:2009} which performs electronic transactions without the involvement of the third party. The term \SContract{} \cite{Nick:PublicN:journals:1997} has been introduced by Nick Szabo. \emph{Smart contract} is an interface to reduce the computational transaction cost and provides secure relationships on public networks. There exist few paper in the literature that works on safety and security concern of smart contracts. Luu et al. \cite{Luu+:DIC:CCS:2015} addresses the waste part of the computational effort by miner that can be utilized and lead to award the incentives.  Delmolino et al.\cite{Delmolino+:SSTCSC:FC:2016} document presents the common pitfall made while designing a secure smart contract. Nowadays, ethereum \cite{ethereum} is one of the most popular smart contract platform which supports a built-in Turing-complete programming language. Ethereum virtual machine (EVM) uses Solidity \cite{Solidity} programming language. Luu et al.\cite{Luu+:MSC:CCS:2016} addresses several security problems and proposed an enhanced mechanism to make the ethereum smart contracts less vulnerable.

Sergey et al. \cite{SergeyandHobor:ACP:2017} elaborates a new perspective between smart contracts and concurrent objects. Zang et al. \cite{ZangandZang:ECSC:WBD:2018} uses any concurrency control mechanism for concurrent miner which delays the read until the corresponding writes to commit and ensures conflict-serializable schedule. Basically, they proposed concurrent validators using MVTO protocol with the help of write sets provided by the concurrent miner. Dickerson et al. \cite{Dickerson+:ACSC:PODC:2017} introduces a speculative way to execute smart contracts by using concurrent miner and concurrent validators. They have used pessimistic software transactional memory systems (STMs) to execute concurrent smart contracts which use rollback if any inconsistency occurs and prove that schedule generated by concurrent miner is \emph{serializable}. We proposed an efficient framework for concurrent execution of the smart contracts using optimistic software transactional memory systems. So, the updates made by a transaction will be visible to shared memory only on commit hence, rollback is not required. Our approach ensures correctness criteria as opacity \cite{GuerKap:Opacity:PPoPP:2008} which considers aborted transactions as well because it read correct values.

Weikum et al. \cite{WeiVoss:TIS:2002:Morg} proposed concurrency control techniques that maintain single-version and multiple versions corresponding to each data-object. STMs \cite{HerlMoss:1993:SigArch,ShavTou:1995:PODC} are alternative to locks for addressing synchronization and concurrency issues in multi-core systems. STMs are suitable for the concurrent executions of smart contracts without worrying about consistency issues. Single-version STMs protocol store single version corresponding to each data-object as BTO STM. It identifies the conflicts between two transactions at run-time and abort one of them and retry again for the aborted transaction. Kumar et al. \cite{Kumar+:MVTO:ICDCN:2014} observe that storing multiple versions corresponding to each data-object reduces the number of aborts and provides greater concurrency that leads to improving the throughput.



\cmnt{
\vspace{1mm}
\noindent
\textbf{Related Work:} The first \emph{blockchian} concept has been given by Satoshi Nakamoto in 2009 \cite{Nakamoto:Bitcoin:2009}. He proposed a system as bitcoin \cite{Nakamoto:Bitcoin:2009} which performs electronic transactions without the involvement of the third party. The term \SContract{} \cite{Nick:PublicN:journals:1997} has been introduced by Nick Szabo. \emph{Smart contract} is an interface to reduce the computational transaction cost and provides secure relationships on public networks. %There exist few paper in the literature that works on safety and security concern of smart contracts. Luu et al. \cite{Luu+:DIC:CCS:2015} addresses the waste part of computational effort by miner that can be utilized and lead to award the incentives.  Delmolino et al.\cite{Delmolino+:SSTCSC:FC:2016} document presents the common pitfall made by students while designing a secure smart contract. 
Nowadays, ethereum \cite{ethereum} is one of the most popular smart contract platform which supports a built-in Turing-complete programming language such as Solidity \cite{Solidity}.% Luu et al.\cite{Luu+:MSC:CCS:2016} addresses several security problems and proposed an enhanced mechanism to make the ethereum smart contracts less vulnerable.

Sergey et al. \cite{SergeyandHobor:ACP:2017} elaborates a new perspective between smart contracts and concurrent objects. Zang et al. \cite{ZangandZang:ECSC:WBD:2018} uses any concurrency control mechanism for concurrent miner which delays the read until the corresponding writes to commit and ensures conflict-serializable schedule. Basically, they proposed concurrent validators using MVTO protocol with the help of write sets provided by concurrent miner. Dickerson et al. \cite{Dickerson+:ACSC:PODC:2017} introduces a speculative way to execute smart contracts by using concurrent miner and concurrent validators. They have used pessimistic software transactional memory systems (STMs) to execute concurrent smart contracts which use rollback, if any inconsistency occurs and prove that schedule generated by concurrent miner is \emph{serializable}. We propose an efficient framework for the execution of concurrent smart contracts using optimistic software transactional memory systems. So, the updates made by a transaction will be visible to shared memory only on commit hence, rollback is not required. Our approach ensures correctness criteria as opacity \cite{GuerKap:Opacity:PPoPP:2008, tm-book} by Guerraoui \& Kapalka, which considers aborted transactions as well because it read correct values.

%Weikum et al. \cite{WeiVoss:TIS:2002:Morg} proposed concurrency control techniques that maintain single-version and multiple versions corresponding to each data-object. STMs \cite{HerlMoss:1993:SigArch,ShavTou:1995:PODC} are alternative to locks for addressing synchronization and concurrency issues in multi-core systems. STMs are suitable for the concurrent executions of smart contracts without worrying about consistency issues. Single-version STMs protocol store single version corresponding to each data-object as BTO STM. It identifies the conflicts between two transactions at run-time and abort one of them and retry again for aborted transaction. Kumar et al. \cite{Kumar+:MVTO:ICDCN:2014} observe that storing multiple versions corresponding to each data-object reduces number of aborts and provides greater concurrency that leads to improving the throughput.
}

==> Arxiv version Archit pdp-19-bc (H space) (copy)/macros.tex <==
% comment a region

\newcommand{\punt}[1]{}
\newcommand{\cmnt}[1]{}


% a word should not be broken across lines
\newcommand{\nosplit}{\linebreak}

% no hyphenation
\def\nohyphens{\hyphenpenalty=10000\exhyphenpenalty=10000}

% ~ character
\newcommand{\tilda}{\symbol{126}}

% useful mathematical symbols

\newcommand{\ang}[1]{\langle #1 \rangle}
\newcommand{\Ang}[1]{\Big\langle #1 \Big\rangle}
\newcommand{\ceil}[1]{\lceil #1 \rceil}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}


% quantifiers
\newcommand{\myforall}[3]{\ang{\forall \: #1 : #2 : #3 }}
\newcommand{\myexists}[3]{\ang{\exists \: #1 : #2 : #3 }}
\newcommand{\mynexists}[3]{\ang{\nexists \: #1 : #2 : #3 }}
\newcommand{\Myforall}[3]{\Ang{\forall \: #1 : #2 : #3 }}
\newcommand{\Myexists}[3]{\Ang{\exists \: #1 : #2 : #3 }}
\newcommand{\Mynexists}[3]{\Ang{\nexists \: #1 : #2 : #3 }}


% for formally defining a notion
% \newcommand{\defined}{\;\;\stackrel{\triangle}{=}\;\;}
\newcommand{\defined}{\;\;\triangleq\;\;}


% mathematical implications

%\renewcommand{\implies}{\Rightarrow}
\newcommand{\follows}{\Leftarrow}

% miscellaenous
\newcommand{\myspace}{\hspace*{0.0in}}
\newcommand{\halflinespacing}{\vspace*{0.5em}}
\newcommand{\greaterlinespacing}{\vspace*{0.75em}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% keywords for pseudocode

\newcommand{\myif}{\textbf{if}}
\newcommand{\mythen}{\textbf{then}}
\newcommand{\myelse}{\textbf{else}}
\newcommand{\myendif}{\textbf{endif}}
\newcommand{\myor}{\textbf{or}}
\newcommand{\myand}{\textbf{and}}
\newcommand{\mynot}{\textbf{not}}

%% various theorem environments
%% Commented out because they are already defined in llncs file %%
%% Decommented out because they are not defined in sigplan class %%

%\newtheorem{theorem}{Theorem}
%\renewcommand{\thetheorem}{\arabic{theorem}}

%\newtheorem{lemma}[theorem]{Lemma}
%\newtheorem{corollary}[theorem]{Corollary}
%\newtheorem{proposition}[theorem]{Proposition}
%\newtheorem{property}[theorem]{Property}
%\newtheorem{definition}[theorem]{Definition}

%\renewtheorem{property}[theorem]{Property}

%\newtheorem{definition}{Definition}
%\renewcommand{\thedefinition}{\arabic{definition}}

%\newtheorem{property}{Property}
%\renewcommand{\theproperty}{\arabic{property}}

%\newtheorem{observation}[theorem]{Observation}
%\renewcommand{\theobservation}{\arabic{observation}}

%\newtheorem{example}{Example}
%\renewcommand{\theexample}{\arabic{example}}

%\newtheorem{assume}{Assumption}
%\renewcommand{\theassume}{\arabic{assume}}

%\newtheorem{remark}{Remark}
%\renewcommand{\theremark}{\arabic{remark}}

%\newtheorem{axiom}[theorem]{Proposition}
%\renewcommand{\theaxiom}{\arabic{axiom}}

%\newtheorem{invariant}[theorem]{Invariant}

%\renewcommand{\theequation}{\arabic{equation}}

%-----------------Theorem Notations Defined by Petr ---------------------------------------------------------------------------------------------------------
%% Defined by Petr
\newtheorem{theorem}{Theorem}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{property}[theorem]{Property}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{result}[theorem]{Result}
\newtheorem{requirement}[theorem]{Requirement}
%\newtheorem{acknowledgement}[theorem]{Acknowledgement}
%\newtheorem{algorithm}[theorem]{Algorithm}
%\newtheorem{case}[theorem]{Case}
%\newtheorem{claim}[theorem]{Claim}
%\newtheorem{explanation}[theorem]{Explanation}
%\newtheorem{fact}[theorem]{Fact}
% \newtheorem{conclusion}[theorem]{Conclusion}
% \newtheorem{condition}[theorem]{Condition}
%\newtheorem{conjecture}[theorem]{Conjecture}
% \newtheorem{criterion}[theorem]{Criterion}
%\newtheorem{definition}[theorem]{Definition}
% \newtheorem{example}[theorem]{Example}
% \newtheorem{exercise}[theorem]{Exercise}
%\newtheorem{lemma}[theorem]{Lemma}
% \newtheorem{notation}[theorem]{Notation}
% \newtheorem{problem}[theorem]{Problem}
%\newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{remark}[theorem]{Remark}
% \newtheorem{solution}[theorem]{Solution}
% \newtheorem{summary}[theorem]{Summary}
%\newtheorem{observation}[theorem]{Observation}
\newenvironment{proof}[1][Proof]{\noindent\textbf{#1.} }{} %\rule{0.5em}{0.5em}\\}
%\newenvironment{proofsketch}[1][Proof sketch]{\noindent\textbf{#1.} }{\hfill $\Box$\\[2mm]} %\rule{0.5em}{0.5em}\\}
%\newenvironment{reptheorem}[1][Theorem]{\noindent\textbf{#1}}{}

%------------------------------------------------------------------------------------------------------------------------------

% various references
\newcommand{\chapref}[1]{Chapter~\ref{chap:#1}}
\newcommand{\secref}[1]{Section~\ref{sec:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\stref}[1]{step~\ref{step:#1}}
\newcommand{\thmref}[1]{Theorem~\ref{thm:#1}}
\newcommand{\lemref}[1]{Lemma~\ref{lem:#1}}
%\newcommand{\corref}[1]{Corollary~\ref{cor:#1}}
\newcommand{\axmref}[1]{Proposition~\ref{axm:#1}}
\newcommand{\defref}[1]{Definition~\ref{def:#1}}
\newcommand{\eqnref}[1]{Eqn(\ref{eq:#1})}
\newcommand{\eqvref}[1]{Equivalence~(\ref{eqv:#1})}
\newcommand{\ineqref}[1]{Inequality~(\ref{ineq:#1})}
%\newcommand{\invref}[1]{(\ref{inv:#1})}
\newcommand{\exref}[1]{Example~\ref{ex:#1}}
\newcommand{\propref}[1]{Property~\ref{prop:#1}}
\newcommand{\obsref}[1]{Observation~\ref{obs:#1}}
\newcommand{\asmref}[1]{Assumption~\ref{asm:#1}}
\newcommand{\thref}[1]{Thread~\ref{th:#1}}
\newcommand{\trnref}[1]{Transaction~\ref{trn:#1}}

%\newcommand{\lineref}[1]{Line~\ref{lin:#1}}
\newcommand{\algoref}[1]{{Algorithm \ref{alg:#1}}}
\newcommand{\subsecref}[1]{SubSection~\ref{subsec:#1}}
\newcommand{\subsubsecref}[1]{SubSubSection~\ref{subsubsec:#1}}

\newcommand{\apnref}[1]{Appendix~\ref{apn:#1}}
\newcommand{\invref}[1]{Invariant~\ref{inv:#1}}

\newcommand{\Chapref}[1]{Chapter~\ref{chap:#1}}
\newcommand{\Secref}[1]{Section~\ref{sec:#1}}
\newcommand{\Figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\Tabref}[1]{Table~\ref{tab:#1}}
\newcommand{\Stref}[1]{Step~\ref{step:#1}}
\newcommand{\Thmref}[1]{Theorem~\ref{thm:#1}}
\newcommand{\Lemref}[1]{Lemma~\ref{lem:#1}}
\newcommand{\Corref}[1]{Corollary~\ref{cor:#1}}
\newcommand{\Axmref}[1]{Proposition~\ref{axm:#1}}
\newcommand{\Defref}[1]{Definition~\ref{def:#1}}
\newcommand{\Eqref}[1]{(\ref{eq:#1})}
\newcommand{\Eqvref}[1]{Equivalence~(\ref{eqv:#1})}
\newcommand{\Ineqref}[1]{Inequality~(\ref{ineq:#1})}
\newcommand{\Exref}[1]{Example~\ref{ex:#1}}
\newcommand{\Propref}[1]{Property~\ref{prop:#1}}
\newcommand{\Obsref}[1]{Observation~\ref{obs:#1}}
\newcommand{\Asmref}[1]{Assumption~\ref{asm:#1}}

\newcommand{\Lineref}[1]{Line~\ref{lin:#1}}
\newcommand{\Algoref}[1]{{\sf Algo$_{\ref{algo:#1}}$}}

\newcommand{\Apnref}[1]{Section~\ref{apn:#1}}
\newcommand{\Invref}[1]{Invariant~\ref{inv:#1}}


% environment for writing a proof

%\newcommand{\proof}[1][]{\noindent{\bf\boldmath
%                          P\hspace{-0.25ex}roof{#1}\/:\unboldmath}\hspace*{0.5em}}


%\newcommand{\theqed}{$\Box$}

%\newcommand{\qed}{\hspace*{\fill}\theqed\\\vspace*{-0.5em}}

% In case the proof is immediately followed by the start of a new section

\newcommand{\nsqed}{\hspace*{\fill} \theqed}


% End of example

\newcommand{\eoe}{\qed}

% Renews the footnote command
\renewcommand{\thefootnote}{\alph{footnote}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Definitions by Petr 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\lf{\tiny}
\def\rrnnll{\setcounter{linenumber}{0}}
\def\nnll{\refstepcounter{linenumber}\lf\thelinenumber}
%\newcounter{linenumber}
%\newenvironment{algorithmfig}{\hrule\vskip 3mm}{ \vskip 3mm \hrule }

\def\P{\ensuremath{\mathcal{P}}}
\def\DP{\ensuremath{\Diamond\mathcal{P}}}
\def\DS{\ensuremath{\Diamond\mathcal{S}}}
\def\T{\ensuremath{\mathcal{T}}}
\def\Time{\mathbb{T}}
\def\S{\ensuremath{\mathcal{S}}}
\def\D{\ensuremath{\mathcal{D}}}
\def\W{\ensuremath{\mathcal{W}}}
\def\A{\ensuremath{\mathcal{A}}}
\def\B{\ensuremath{\mathcal{B}}}
\def\F{\ensuremath{\mathcal{F}}}
\def\R{\ensuremath{\mathcal{R}}}
\def\H{\ensuremath{\mathcal{H}}}
%\def\N{\ensuremath{\mathcal{N}}}
\def\N{\ensuremath{\mathbb{N}}}
\def\I{\ensuremath{\mathcal{I}}}
\def\O{\ensuremath{\mathcal{O}}}
\def\Q{\ensuremath{\mathcal{Q}}}
\def\K{\ensuremath{\mathcal{K}}}
\def\L{\ensuremath{\mathcal{L}}}
\def\M{\ensuremath{\mathcal{M}}}
\def\V{\ensuremath{\mathcal{V}}}
\def\E{\ensuremath{\mathcal{E}}}
\def\C{\ensuremath{\mathcal{C}}}
%\def\T{\ensuremath{\mathcal{T}}}
\def\X{\ensuremath{\mathcal{X}}}
\def\Y{\ensuremath{\mathcal{Y}}}
\def\Nat{\ensuremath{\mathbb{N}}}
\def\Om{\ensuremath{\Omega}}
\def\ve{\varepsilon}
\def\fd{failure detector}
\def\cfd{\ensuremath{?\P+\DS}}
\def\afd{timeless}
\def\env{\ensuremath{\mathcal{E}}}
%\def\faulty{unreliable}
\def\bounded{one-shot}
\def\cons{\textit{cons}}
\def\val{\textit{val}}
\def\code{\textit{code}}

\def\HSS{\mathit{h}}
\def\argmin{\mathit{argmin}}
\def\proper{\mathit{proper}}
\def\content{\mathit{content}}
\def\Level{\mathit{L}}
\def\Blocked{\mathit{Blocked}}
\def\Set{\mathit{Set}}


\newcommand{\remove}[1]{}

\newcommand{\Wset}{\textit{Wset}}
\newcommand{\Rset}{\textit{Rset}}
\newcommand{\Dset}{\textit{Dset}}
%\newcommand{\T}{$\mathcal{T}$}

%\newcommand{\parts}{\textit{parts}}

\newcommand{\trylock}{\textit{trylock}}
\newcommand{\multitrylock}{\textit{multi-trylock}}
\newcommand{\CAS}{\textit{CAS}}
\newcommand{\mCAS}{\textit{mCAS}}

\def\Nomega{\ensuremath{\neg\Omega}}
\def\Vomega{\ensuremath{\overrightarrow{\Omega}}}

\newcommand{\id}[1]{\mbox{\textit{#1}}}% for identifiers in code
\newcommand{\res}[1]{\mbox{\textbf{#1}}}% reserved words

\newcommand{\ignore}[1]{}

\newcommand{\myparagraph}[1]{\vspace{1mm}\noindent\textbf{#1}}

%------------------------------------------------------------------------------------------------------------------
% Definitions for Weak Consistency paper
%------------------------------------------------------------------------------------------------------------------

\newcommand{\op} {operation}
\newcommand{\termop} {terminal operation}
\newcommand{\nonin} {non-interference}
\newcommand{\perm} {permissive}
\newcommand{\pness} {permissiveness}
\newcommand{\ai} {abort-invisible}
\newcommand{\ait} {abort-invisiblity}
\newcommand{\vwc} {\textit{VWC}}
\newcommand{\lo} {\textit{LO}}
\newcommand{\clo} {\textit{CLO}}
\newcommand{\svlo} {\textit{CLO}}
\newcommand{\svsls} {\textit{CLO}}

\newcommand{\sts} {SS}
\newcommand{\comm}[1] {\textit{committed(#1)}}
\newcommand{\aborted}[1] {\textit{aborted}(#1)}
\newcommand{\txns}[1] {\textit{txns}(#1)}
\newcommand{\forceCom}[2] {$#1^{#2,C}$}
\newcommand{\remSub}[2] {$#2_{-#1}$}
\newcommand{\permfn}[1] {Perm(#1)}
\newcommand{\nifn}[1] {\textit{NI}(#1)}
\newcommand{\prevA}[2] {\textit{IncAbort}(#1, #2)}
\newcommand{\prevC}[2] {\textit{priorCommit}(#1, #2)}
\newcommand{\evts}[1] {evts(#1)}
\newcommand{\ssch} {sub-history\xspace}
\newcommand{\sschs} {sub-historie\xspaces}
\newcommand{\serial} {serial\xspace}
\newcommand{\serialc} {serial criterion\xspace}
\newcommand{\svserial} {sv-serial\xspace}
\newcommand{\svsc} {sv-serial criterion\xspace}

\newcommand{\wrt}[2] {#2.wTrans(#1)}
\newcommand{\wtrans} {wTrans}
\newcommand{\cwrt}[2] {#2.cwTrans(#1)}
\newcommand{\cwtrans} {cwTrans}

\newcommand{\valid} {valid}
\newcommand{\validity} {validity}
\newcommand{\legal} {legal}
\newcommand{\legality} {legality}
\newcommand{\leg}[1] {#1\text{-}legal}

\newcommand{\tobj} {\emph{t-object}}
\newcommand{\gchist} {\textit{gComHist}}
\newcommand{\lchist} {\textit{lComHist}}
\newcommand{\thist} {\textit{tHist}}
\newcommand{\gchlock} {\textit{gLock}}
\newcommand{\gseqn}{\textit{gSeqNum}}
\newcommand{\cseq} {\textit{commitSeqNum}}
\newcommand{\rseq} {\textit{readSeqNum}}
\newcommand{\lseq} {\textit{lseq}}
%\newcommand{\tryc} {\textit{tryC}}
%\newcommand{\trya}{\textit{tryA}}
\newcommand{\rvar} {\textit{readVar}}
\newcommand{\rop} {\textit{rop}}
\newcommand{\wvar} {\textit{writeVar}}
\newcommand{\wop} {\textit{wop}}
\newcommand{\cvar} {\textit{comVar}}
\newcommand{\cop} {\textit{cop}}

\newcommand{\co} {CO\xspace}
\newcommand{\opq} {opaque\xspace}
\newcommand{\opaq}[1] {#1\text{-}opaque\xspace}
%\newcommand{\opaq}[1] {#1-opaque}
\newcommand{\opaty}[1] {#1\text{-}opacity\xspace}
%\newcommand{\opaty}[1] {#1-opacity}
\newcommand{\opty} {opacity\xspace}
\newcommand{\coop} {co-opaque\xspace}
\newcommand{\coopty} {co-opacity\xspace}

\newcommand{\sble} {serializable\xspace}
\newcommand{\sbty} {serializability\xspace}
\newcommand{\lble} {linearizable\xspace}
\newcommand{\lbty} {linearizability\xspace}


% Definitions for proof in this paper
\newcommand{\pref}[2] {#2.prefix(#1)}
\newcommand{\cpref}[2] {#2.comPrefix(#1)}
\newcommand{\compref} {comPrefix\xspace}

% Definitions needed for Garbage Collection
\newcommand{\liveset} {liveSet\xspace}
\newcommand{\primary} {primary\xspace}
\newcommand{\glset} {gIncSet\xspace}
\newcommand{\waits} {waitSet\xspace}
\newcommand{\dset} {dependSet\xspace}
\newcommand{\sstate} {system-state\xspace}
\newcommand{\obsolete} {obsolete\xspace}

%------------------------------------------------------------------------------------------------------------------
% Definitions for Multiversion timestamp ordering protocol paper
%------------------------------------------------------------------------------------------------------------------
\newcommand{\mvs} {multi-version STM}

\newcommand{\tseq} {t-sequential\xspace}
\newcommand{\opg}[2] {OPG(#1, #2)}
\newcommand{\ord}[1] {ord(#1)}
\newcommand{\ordfn} {ord}
\newcommand{\mv} {mv}
\newcommand{\rf} {rf}
\newcommand{\rt} {rt}
\newcommand{\mvto} {MVTO\xspace}
\newcommand{\bto} {BTO\xspace}
\newcommand{\memop} {memory operation\xspace}

\newcommand{\cc} {correctness-criterion\xspace}


\newcommand{\readi} {\emph{$read_i$}\xspace}
\newcommand{\cl} {\emph{confList}\xspace}
\newcommand{\writei} {stm\_write\xspace}
\newcommand{\tryci} {stm\_tryC\xspace}
%\newcommand{\tryc} {\emph{tryC}\xspace}
\newcommand{\tryc} {STM.tryC\xspace}
\newcommand{\tryai} {stm\_tryA\xspace}
%\newcommand{\trya} {tryA}
\newcommand{\trya} {STM.tryA}
\newcommand{\ok} {stm\_ok}

%\newcommand{\read} {stm\_read}
%\newcommand{\write} {stm\_write}
%\newcommand{\trya} {stm\_tryA}
%\newcommand{\ok} {stm\_ok}

\newcommand{\tcntr} {\emph{tCounter}\xspace}
\newcommand{\shl} {\emph{shl}\xspace}
\newcommand{\mr} {\emph{max\_r}\xspace}
\newcommand{\mw} {\emph{max\_w}\xspace}
\newcommand{\cminer} {Concurrent Miner\xspace}
\newcommand{\cvalidator} {Concurrent Validator\xspace}
\newcommand{\conminer} {\emph{concurrent miner}\xspace}
\newcommand{\convalidator} {\emph{concurrent validator}\xspace}
\newcommand{\Conminer} {\emph{Concurrent Miner}\xspace}
\newcommand{\Convalidator} {\emph{Concurrent Validator}\xspace}
\newcommand{\ConValidator} {\emph{Concurrent validator}\xspace}
\newcommand{\CG} {\emph{Conflict Graph}\xspace}
\newcommand{\cgraph} {\emph{conflict graph}\xspace}
\newcommand{\Cgraph} {\emph{Conflict graph}\xspace}
\newcommand{\bg} {block graph\xspace}
\newcommand{\aul} {\emph{auList[]}\xspace}
\newcommand{\confg} {\emph{confGraph}\xspace}
\newcommand{\gconfl} {\emph{getConfList}\xspace}
\newcommand{\vp} {\emph{vPred}\xspace}
\newcommand{\vc} {\emph{vCurr}\xspace}
\newcommand{\vn} {\emph{vNext}\xspace}
\newcommand{\ep} {\emph{ePred}\xspace}
\newcommand{\ec} {\emph{eCurr}\xspace}
\newcommand{\en} {\emph{eNext}\xspace}
\newcommand{\vl} {\emph{vList}\xspace}
\newcommand{\el} {\emph{eList}\xspace}
\newcommand{\inc} {\emph{inCnt}\xspace}
\newcommand{\txlog} {\emph{txlog}\xspace}
\newcommand{\adde} {\emph{addEdge}\xspace}
\newcommand{\addv} {\emph{addVert}\xspace}
\newcommand{\egn} {\emph{eNode}\xspace}
\newcommand{\vgn} {\emph{vNode}\xspace}
\newcommand{\enode} {\emph{eNode}\xspace}
\newcommand{\vnode} {\emph{vNode}\xspace}
\newcommand{\searchl} {\emph{searchLocal}\xspace}
\newcommand{\searchg} {\emph{searchGlobal}\xspace}
\newcommand{\bc} {blockchain\xspace}
\newcommand{\BC} {Blockchain\xspace}
\newcommand{\scontract} {smart contract\xspace}
\newcommand{\SContract} {smart contract\xspace}
\newcommand{\Scontract} {Smart contract\xspace}
\newcommand{\au} {atomic-unit\xspace}
\newcommand{\miner} {miner\xspace}
\newcommand{\validator} {validator\xspace}
\newcommand{\Miner} {miner\xspace}
\newcommand{\Validator} {validator\xspace}
\newcommand{\exec} {\emph{executeCode}\xspace}
\newcommand{\hb} {happens-before\xspace}

\newcommand{\nc} {\emph{nCount}\xspace}
\newcommand{\gn} {\emph{gNode}\xspace}
\newcommand{\vt} {\emph{vTail}\xspace}
\newcommand{\vh} {\emph{vHead}\xspace}
\newcommand{\eh} {\emph{eHead}\xspace}
\newcommand{\et} {\emph{eTail}\xspace}
\newcommand{\tl} {\emph{thLog}\xspace}
\newcommand{\cachel} {\emph{cacheList}\xspace}
\newcommand{\vmain} {\emph{validatorMain}\xspace}
\newcommand{\opt} {\emph{Opt}\xspace}
\newcommand{\vtuple} {\emph{v\_tuple}\xspace}
\newcommand{\dtuple} {\emph{d\_tuple}\xspace}
\newcommand{\ctuple} {\emph{c\_tuple}\xspace}
\newcommand{\livel} {liveList\xspace}
\newcommand{\begtrans} {\emph{begin}\xspace}
\newcommand{\checkv} {check\_versions\xspace}
\newcommand{\init} {\emph{initialize}\xspace}
\newcommand{\find} {find\_lts\xspace}
\newcommand{\instup} {ins\_tuple\xspace}
\newcommand{\remid} {removeId\xspace}
\newcommand{\gc} {gc\xspace}

\newcommand{\vwrite} {valWrite\xspace}
\newcommand{\valw}[2] {#2.valWrite(#1)}
\newcommand{\lastw} {lastWrite}
\newcommand{\lwrite}[2] {#2.lastWrite(#1)}
\newcommand{\lastwr} {writerTrans\xspace}
\newcommand{\cg}[1] {CG(#1)}

\newcommand{\mvve} {MVVE\xspace}
\newcommand{\vie} {VE\xspace}
\newcommand{\ce} {CE\xspace}

\newcommand{\locko} {lockOrder\xspace}
\newcommand{\lopg}[1] {#1.lockOpGraph\xspace}
\newcommand{\aco} {accessOrder\xspace}
\newcommand{\seq}[2] {linearize(#2, #1)}
\newcommand{\stl}[3] {#3.stl(#1, #2)}
\newcommand{\stln} {stl}
\newcommand{\lts}[3] {#3.lts(#1, #2)}
\newcommand{\ltsn} {lts}
\newcommand{\vli}[3] {#3.vlist\_index(#1, #2)}
\newcommand{\hlive}[1] {liveTrans(#1)\xspace}

\newcommand{\mvperm} {mv-permissive\xspace}
\newcommand{\mvpness} {mv-permissiveness\xspace}

\newcommand{\gen}[1] {gen(#1)}
\newcommand{\mlive} {maxLiveSet}
\newcommand{\maxl}[1] {maxLiveSet(#1)}
\newcommand{\prefs}[1] {prefixSet(#1)}


% Definitions for the pseudocode
%\algrenewcommand{\algorithmiccomment}[1]{\hskip3em$//$ #1}
%\algrenewcommand{\algorithmiccomment}[1]{$//$ #1}
\newcommand{\rs}{rset\xspace}
\newcommand{\ws}{wset\xspace}


%\newcommand{\init} {init\xspace}
%\newcommand{\begt} {tbegin\xspace}
%\newcommand{\tread} {stm\text{-}read\xspace}
%\newcommand{\twrite} {stm\text{-}write\xspace}

\newcommand{\begt} {STM.begin\xspace}
\newcommand{\tread} {STM.read\xspace}
\newcommand{\twrite} {STM.write\xspace}

%\newcommand{\tryc} {tryC\xspace}
%\newcommand{\trya} {tryA\xspace}
\newcommand{\tmth} {stm\text{-}method\xspace}
\newcommand{\commit}{\mathcal{C}}
\newcommand{\abort}{\mathcal{A}}
%\newcommand{\op} {operation\xspace}
\newcommand{\mth} {method\xspace}


\newcommand {\incomp}[1] {#1.incomp}
\newcommand {\live}[1] {#1.live}

\newcommand{\shist}[2] {#2.subhist(#1)\xspace}
\newcommand{\subhist} {subhist\xspace}
\newcommand{\subhs} {subhistSet\xspace}
\newcommand{\shset}[1] {#1.subhistSet\xspace}


==> Arxiv version Archit pdp-19-bc (H space) (copy)/objective.tex <==
\section{Requirements of Concurrent Miner, Validator and Block Graph}
\label{sec:req-miner_val}

This section describes the requirements of concurrent miner, validator and block graph to ensure correct concurrent execution of the \scontract transactions. 

%\todo{In one of the sections below, bring the ideas of MVE, VE \& CE.}

\subsection{Requirements of the Concurrent Miner}
The miner process invokes several threads to concurrently execute the \scontract transactions or \au{s}. With the proposed optimistic execution approach, each miner thread invokes an \au as a transaction. %It is important to ensure that the concurrent execution is \emph{correct}. 

The miner should ensure the correct concurrent execution of the smart contract transactions. The incorrect concurrent execution (or consistency issues) may occur when concurrency involved. Any inconsistent read may leads system to divide by zero, infinite loops, crash failure etc. All smart contract transactions take place within a virtual machine \cite{Dickerson+:ACSC:PODC:2017}. %Virtual machine environment can get rid of the issues of inconsistent read while executing the smart contract transactions sequentially. 
When miner executes the smart contract transactions concurrently on the virtual machine then infinite loop and inconsistent read may occur. So, to ensure the correct concurrent execution, the miner should satisfy the correctness-criterion as opacity \cite{GuerKap:Opacity:PPoPP:2008}.

To achieve better efficiency, sometimes we need to adapt the non-virtual machine environment which necessitates with the safeguard of transactions. There as well miner needs to satisfies the correctness-criterion as opacity to ensure the correct concurrent execution of smart contract transactions. %Opacity assures that all the transactions read consistent values including aborted transactions as well. 

%In non-virtual machine environment, any inconsistent read may leads to divide by zero, infinite loops, crash failure of concurrent miner etc. So, the correct concurrent execution by miner should ensures opacity which says all the transactions read consistent values including aborted transactions as well. % The concurrent execution of the \scontract transactions of a block by the validators which although is highly desirable can further complicate the situation. 
\begin{requirement}
	Any history $H_m$ generated by concurrent miner should satisfy opacity.
\end{requirement}
\cmnt{
\begin{proof}
	Here, miner executes the smart contract concurrently with the help of optimistic STM protocols (BTO and MVTO). Internally, BTO and MVTO \cite{Kumar+:MVTO:ICDCN:2014} protocol ensures opacity. So, history $H_m$ generated Concurrent miner satisfies opacity.
\end{proof}
}

%Concurrent miner provides $BG$ to concurrent validators to ensure the correct output by validators. After that concurrent validator apply topological sort on $BG$ and generates a history $H_v$.

%Once a concurrent miner proposes a block, then validator re-executes the same set of transactions concurrently to validate it. But during the concurrent execution, suppose the validator execute two conflicting transactions in a different order from what was executed by the miner. Thus the serialization order of the miner is different from the validator. Then this can result in the validator obtaining a different final state than what was obtained by the miner. Thus the validator may incorrectly reject the block although it is valid. 

Concurrent miner maintains a BG and provides it to concurrent validators which ensures the dependency order among the conflicting transactions. As we discussed in \secref{intro}, if concurrent miner will not maintain the BG then a valid block may get rejected by the concurrent validator. %BG helps to achieve the same final state by concurrent validators as concurrent miner.


\subsection{Requirements of the Concurrent Validator}
The correct concurrent execution by validator should be equivalent to some serial execution. The serial order can be obtained by applying the topological sort on the BG provided by the concurrent miner. BG gives partial order among the transactions while restricting the dependency order same as the concurrent miner. So validator executes those transactions concurrently which are not having any dependency among them with the help of BG. Validator need not have to worry about any concurrency control issues because BG ensures conflicting transactions never execute concurrently.


\subsection{Requirements of the Block Graph}

As explained above, the miner generates a BG to capture the dependencies between the smart contract transactions which is used by the validator to concurrently execute the transactions again later. The validator executes those transactions concurrently which do not have any path (implying dependency) between them. Thus the execution by the validator is  given by a topological sort on the BG. 

Now it is imperative that the execution history generated by the validator, $H_v$ is `equivalent' to the history generated by the miner, $H_m$. The precise equivalence depends on the STM protocol followed by the miners and validators. If the miner uses Multi-version STM such as MVTO then the equivalence between $H_v$ and $H_m$ is \mvve. In this case, the graph generated by the miner would be multi-version serialization graph \cite[Chap. 5]{WeiVoss:TIS:2002:Morg}. 

On the other hand, if the miner uses single version STM such as BTO then the equivalence between $H_v$ and $H_m$ is view-equivalence (\vie) which can be approximated by conflict-equivalence (\ce). Hence, in this case, the graph generated by the miner would be conflict graph \cite[Chap. 3]{WeiVoss:TIS:2002:Morg}. 

%In order to improve the efficiency of concurrent validator, we consider $BG$ which allow to execute the transactions concurrently without abort.


%The correct concurrent validator execution obtains a total order among the transactions. The way, we have done the concurrent validators need not to worry about concurrency control issues.

%\subsection{Requirements of the Block Graph}
\cmnt{
Block graph ensures view equivalence between the histories of the concurrent miners and validators. During the concurrent execution of miner using STM\_BTO protocol, conflict graph (same as BG) captures the view equivalence between the histories of the concurrent miners and validators while maintaining single-version corresponding to each data-objects. We can use the STMs for the concurrent execution by validators but aborts will be there. In order to improve the efficiency of concurrent validator, we consider $BG$ which allow to execute the transactions concurrently without abort. Consider the history $H_m$ generated by STM\_BTO protocol and constructs $BG$ in which each committed transaction $T_i$ consider as vertices and edges between them as follows:
\begin{itemize}
\item r-w: If $T_j$ writes $x$ after read by $T_i$ in $H_m$, then there is an edge from $v_i$ to $v_j$. %Note that in order for this to happen, $T_i$ must have committed before $T_j$ and $c_i$ $<_{H_m}$ $w_j(x)$. 
This set of edges are referred to as r-w.
%$T_i$ reads $x$ from $T_k$, after that $T_j$ writes on $x$ data-object then r-w edge will be from $T_i$ to $T_j$.  
\item w-r: If $T_j$ reads $x$ from $T_i$ in $H_m$, then there is an edge from $v_i$ to $v_j$. Note that in order for this to happen, $T_i$ must have committed before $T_j$ and $c_i$ $<_{H_m}$ $r_j(x)$. This set of edges are referred to as w-r.
%If $T_i$ reads $x$ from the value written by $T_j$ then w-r edge will be from $T_i$ to $T_j$. 
\item w-w: If $T_j$ writes to $x$ after written by $T_i$ in $H_m$, then there is an edge from $v_i$ to $v_j$. Note that in order for this to happen, $T_i$ must have committed before $T_j$ and $c_i$ $<_{H_m}$ $w_j(x)$. This set of edges are referred to as w-w.
%If $T_i$ writes into $x$ before written by $T_j$ then w-w edge will be from $T_i$ to $T_j$. 
\item \rt(real-time) edges: If $T_j$ starts after commit of $T_i$ in $H_m$, then there is an edge from $v_i$ to $v_j$. This set of edges are referred to as $\rt(H_m)$.
\end{itemize}

Whereas when we consider the concurrent execution of miner using STM\_MVTO protocol which stores multiple version corresponding to each data-objects, conflict graph can be restrictive. So, we consider Multi-Version Serialization Graph, MVSG $(H_m,\ll)$ for a given version order of history $H_m$ as follows to ensure the multi-version view equivalence between the histories of the concurrent miners $H_m$ and validators $H_v$:
\begin{enumerate}
\item \textit{\rt}(real-time) edges: If $T_i$ commits before $T_j$ starts in $H_m$, then there is an edge from $v_i$ to $v_j$. This set of edges are referred to as $\rt(H_m)$.

\item \textit{\rf}(reads-from) edges: If $T_j$ reads $x$ from $T_i$ who has written on $x$ in $H_m$, then there is an edge from $v_i$ to $v_j$. Note that in order for this to happen, $T_i$ must have committed before $T_j$ and $c_i$ $<_{H_m}$ $r_j(x)$. This set of edges are referred to as $\rf(H_m)$.

\item \textit{\mv}(multi-version) edges: The \mv{} edges capture the multi-version relations and is based on the version order. Consider a successful read \op{} $r_k(x,v)$ and the write \op{} $w_j(x,v)$ belonging to transaction $T_j$ such that $r_k(x,v)$ reads $x$ from $w_j(x,v)$ (it must be noted $T_j$ is a committed transaction and $c_j$ $<_{H_m}$ $r_k$). Consider a committed transaction $T_i$ which writes to $x$, $w_i(x, u)$ where $u \neq v$. Thus the versions created $x_i, x_j$ are related by $\ll$. Then, if $x_i \ll x_j$ we add an edge from $v_i$ to $v_j$. Otherwise ($x_j \ll x_i$), we add an edge from $v_k$ to $v_i$. This set of edges are referred to as $\mv(H_m, \ll)$.
\end{enumerate}

\begin{lemma}
	History $H_m$ generated by MVTO protocol and $H_v$ are multi-version view equivalent.
\end{lemma}
}

==> Arxiv version Archit pdp-19-bc (H space) (copy)/pm.tex <==
\section{Proposed Mechanism}
\label{sec:pm}
This section presents the methods of lock-free concurrent block graph library followed by concurrent execution of smart contract transactions by miner and validator.
\subsection{Lock-free Concurrent Block Graph}
\label{subsec:bg}
\noindent
%Block graph invokes by the concurrent miner and validator. 
\textbf{Data Structure of Lock-free Concurrent Block Graph:} We use \emph{adjacency list} to maintain the block graph BG(V, E) as shown in \figref{confg} (a). Where V is set of vertices (or \vnode{s}) which are stored in the vertex list (or \vl{}) in increasing order of timestamp between two sentinel node \vh{} (-$\infty$) and \vt{} (+$\infty$). Each vertex node (or \vnode) contains $\langle ts = i, AU_{id} = id, \inc{} = 0, \vn{} = nil, \en{} = nil\rangle$. Where $i$ is a unique timestamp (or $ts$) of committed transactions $T_i$. $AU_{id}$ is the $id$ of \au{} which is executed by transaction $T_i$. To maintain the indegree count of each \vnode{} we initialize \inc{} as 0. \vn{} and \en{} initializes as $nil$. 

Here, E is a set of edges which maintains all the conflicts of \vnode{} in the edge list (or \el) as shown in \figref{confg} (a). \el{} stores \enode{s} (or conflicting transaction nodes say $T_j$) in increasing order of timestamp (or $ts$) between two sentinel nodes \eh{} (-$\infty$) and \et{} (+$\infty$). %We keep a conflict edge between the transaction $T_i$ and $T_j$ in block graph which is going from lower $ts$ to higher $ts$ to make the block graph acyclic. Before adding an edge in the \cgraph{} it checks that both the transactions \vnode{s} should be present in the \vl{} at \Lineref{adde2} and \Lineref{adde3}. If \vnode{} is not part of \vl{} then it creates a node and add it to the \vl{} at \Lineref{addv5} with the help of atomic \emph{compare and swap} operation.    
\vspace{-.3cm}
\begin{figure}[H]
	\centering
		\scalebox{.31}{\input{figs/graphs.pdf_t}}
		\centering
		%		\captionsetup{justification=centering}
		% \vspace{-16cm}
		\caption{Pictorial representation of Block Graph}
		\label{fig:confg}
\end{figure}
\vspace{-.4cm}


\cmnt{
\begin{figure*}
	\centering
	\begin{minipage}[b]{0.3\textwidth}
		\scalebox{.31}{\input{figs/graphs.pdf_t}}
		\centering
		%		\captionsetup{justification=centering}
		% \vspace{-16cm}
		\caption{Pictorial representation of Block Graph}
		\label{fig:confg}
	\end{minipage}
	\hfill
	\begin{minipage}[b]{0.5\textwidth}
		%		\captionsetup{justification=centering}
		\scalebox{.32}{\input{figs/cminer.pdf_t}}
		% \vspace{-16cm}
		\centering
		\caption{Execution of Concurrent Miner}
		\label{fig:cminer}
	\end{minipage}   
\end{figure*}
}
%After successful addition of \vnode{s} corresponding to the transactions $T_i$ and $T_j$ in \vl{}, \cgraph{} maintains the conflict edge in \el{}. Lets assume $ts$ of $T_i$ is less then the $ts$ of $T_j$. So conflict edge should go from $T_i$ to $T_j$.
Edge node (or \enode{}) contains $\langle$\emph{ts = j, vref}, \en{} = $nil$ $\rangle$. Here, $j$ is a unique timestamp (or $ts$) of \emph{committed} transaction $T_j$ which is having conflict with $T_i$ and $ts(T_i)$ is less than $ts(T_j)$. To maintain the acyclicity of the BG, we add a conflict edge from lower timestamp transaction to higher timestamp transaction i.e. conflict edge is from $T_i$ to $T_j$ in the BG. \figref{confg} (b) illustrates this using three transactions with timestamp 0, 5, and 10, which maintain the acyclicity while adding an edge from lower to higher timestamp. \emph{Vertex node reference (or vref)} keeps the reference of its own vertex which is present in the \vl. \en{} initializes as $nil$. %After successful addition of \enode{} in the \el{} of \vnode{}, transaction $T_i$ increment the \inc{} of \enode.$vref$ node which is present in the \vl{} at \Lineref{adde8} because $T_j$ is having an incoming edge from $T_i$.  

Block graph generated by the concurrent miner which helps to execute the validator concurrently and deterministically through lock-free graph library methods. Lock-free graph library consists of five methods as follows: \emph{addVert(), addEdge(), searchLocal(), searchGlobal()} and \emph{decInCount()}. 

\noindent
\textbf{Lock-free Graph Library Methods Accessed by Concurrent Miner:} Concurrent miner uses addVert() and addEdge() methods of lock-free graph library to build a BG. When concurrent miner wants to add a node in the BG then first it calls addVert() method. addVert() method identifies the correct location of that node (or \vgn{}) in the \vl{}. If \vgn{} is not part of \vl{} then it creates the node and adds it into \vl{} in lock-free manner with the help of atomic compare and swap operation. %Otherwise, \vgn{} is already present in \vl{}.

After successful addition of \vnode{} in the BG concurrent miner calls addEdge() method to add the conflicting node (or \egn{}) corresponding to \vnode{} in the \el{}. First, addEdge() method identifies the correct location of \egn{} in the \el{} of corresponding \vnode{}. If \egn{} is not part of \el{} then it creates the node and adds it into \el{} of \vnode{} in lock-free manner with the help of atomic compare and swap operation. After successful addition of \enode{} in the \el{} of \vnode{}, it increment the \inc{} of \enode.$vref$ (to maintain the indegree count) node which is present in the \vl{}.



\noindent
\textbf{Lock-free Graph Library Methods Accessed by Concurrent Validator:} Concurrent validator uses searchLocal(), searchGlobal() and decInCount() methods of lock-free graph library. First, concurrent validator thread calls searchLocal() method to identify the source node (having indegree (or \inc) 0) in its local \cachel{} (or thread local memory). If any source node exist in the local \cachel{} with \inc{} 0 then it sets \inc{} field to be -1 atomically to claim the ownership of the node.% to execute the respective AU %., so that other threads will not work on the same node. After that validator thread executes the \au{} corresponding to that source node 
% and compute the other valid state. 

If the source node does not exists in the local \cachel{} then concurrent validator thread calls searchGlobal() method to identify the source node in the BG. If any source node exists in the BG then it will do the same process as done by searchLocal(). After that validator thread calls the decInCount() to decreases the \inc{} of all the conflicting nodes atomically which are present in the \el{} of corresponding source node. While decrementing the \inc{} of each conflicting nodes in the BG, it again checks if any conflicting node became a source node then it adds that node into its local \cachel{} to optimize the search time of identifying the next source node. Due to lack of space, please refer \apnref{apnbg} to get the complete details with the algorithm of lock-free graph library methods. 







%Smart contracts in \bc{} are executed in two different context. First, by multiple \Miner{s} to propose a new block and after that by multiple \Validator{s} to verify the block proposed by \Miner. So, for the efficient execution of \SContract{s} we propose the \conminer{} who run the \SContract{s} concurrently in optimistic manner using \emph{Software Transactional Memory systems} (STMs) and maintains a block graph. Later, we introduce \convalidator{} who run the \SContract{s} concurrently and deterministically with the help of block graph.     

\subsection{Concurrent Miner}
\label{subsec:cminer}
Smart contracts in \bc{} are executed in two different context. First, by \Miner{} to propose a new block and after that by multiple \Validator{s} to verify the block proposed by \Miner. In this subsection, we describe how miner executes the \SContract{s} concurrently. \tikz \node[circle,scale=.5,color=black, fill=pink]{\textbf{1}}; \emph{Concurrent miner} gets the set of transactions from the \emph{distributed shared memory} as shown in \figref{cminer}. Each transaction associated with the functions (or \au{s}) of smart contracts. To run the \SContract{s} concurrently we have faced the challenge to identify the conflicting transactions at run-time because \SContract{} language are Turing-complete. Two transactions are in conflict if they are accessing common shared data-objects and at least one of them perform write operation on it. \tikz \node[circle,scale=.5,color=black, fill=pink]{\textbf{2}}; In \conminer{}, conflicts are identified at run-time with the help of efficient framework provided by optimistic software transactional memory system (STMs). STMs access the shared data-objects called as \tobj{s}. Each shared \tobj{} having initial state (or IS) which modified by the \au{s} and change IS to some other valid state. Eventually, it reaches to final state (or FS) at the end of block creation. As shown in \algoref{cminer}, first, each transaction $T_i$ gets the unique timestamp $i$ from STM.begin() at \Lineref{cminer5}. Then transaction $T_i$ executes the \au{} of \SContract{s}. \emph{Atomic-unit} consists of multiple steps such as $read$ and $write$ on shared \tobj{s} as $x$. Internally, these $read$ and $write$ steps are handled by the STM.read() and STM.write(), respectively. At \Lineref{cminer9}, if current \au{} step (or curStep) is $read(x)$ then it calls the STM.read(x). Internally, STM.read() identify the shared \tobj{} $x$ from transactional memory (or TM) and validate it. If validation is successful then it gets the value as $v$ at \Lineref{cminer10} and execute the next step of \au{} otherwise re-execute the \au{} if $v$ is $abort$ at \Lineref{cminer11}. 
\vspace{-.3cm}
\begin{figure}[H]
	%		\captionsetup{justification=centering}
	\scalebox{.32}{\input{figs/cminer.pdf_t}}
	% \vspace{-16cm}
	\centering
	\caption{Execution of Concurrent Miner}
	\label{fig:cminer}
\end{figure}
\vspace{-.4cm}

\cmnt{
\begin{figure*}
	\centering
%	\captionsetup{justification=centering}
	\centerline{\scalebox{0.45}{\input{figs/cminer.pdf_t}}}
	\caption{Execution of Concurrent Miner}
	\label{fig:cminer}
\end{figure*}
}
If curStep is $write(x)$ at \Lineref{cminer14} then it calls the STM.write(x). Internally, STM.write() stores the information corresponding to the shared \tobj{} $x$ into transaction local log (or \txlog) in write-set (or $wset_i$) for transaction $T_i$. We use an optimistic approach in which effect of the transaction will reflect onto the TM after the successful STM.tryC(). If validation is successful for all the $wset_i$ of transaction $T_i$ in STM.tryC() i.e. all the changes made by the $T_i$ is consistent then it updates the TM otherwise re-execute the \au{} if $v$ is $abort$ at \Lineref{cminer23}. After successful validation of STM.tryC(), it also maintains the conflicting transaction of $T_i$ into conflict list in TM.
\cmnt{
\begin{figure*}
%	\captionsetup{justification=centering}
	\centerline{\scalebox{0.45}{\input{figs/graphs.pdf_t}}}
	\caption{Pictorial representation of \confg{}, CG}
	\label{fig:confg}
\end{figure*}
}
\cmnt{
Once the transaction commits it stores its conflicts in the form of \CG{}. In order to store the \emph{Conflict Graph} or \confg \emph{(CG(V, E))}, we are maintaining \emph{adjacency list}. In which all the vertices (or \vnode{s}) are stored in the vertex list (or \vl{}) in increasing order of timestamp between the two sentinal node \vh{} (-$\infty$) and \vt{} (+$\infty$). The structure of the vertex node (or \vnode) is as $\langle ts_i, AU_{id}, \inc{}, \vn, \en\rangle$. Where $ts$ is a unique timestamp $i$ of committed transactions $T_i$ assign at the beginning of it. $AU_{id}$ is the $id$ of \au{} which is executed by transaction $T_i$. To maintain the indegree count of each \vnode{} we use \inc{} initialize as 0. \vn{} points to the next vertex of the \vl. For corresponding to each \vnode{}, it maintains all the conflicts in the edge list (\el) as shown in \figref{confg}. \el{} stores \enode{} (or conflicting transaction nodes) belonging to \emph{vNode} stores in increasing order of timestamp (or $ts$) in between the two sentinal nodes \eh{} (-$\infty$) and \et{} (+$\infty$). The structure of \enode{} is as $\langle$\emph{$ts_j$, vref}, \en{} $\rangle$. $ts_j$ is a unique timestamp $j$ of \emph{committed} transaction $T_j$ which had a conflict with $T_i$. \emph{Vertex node reference (or vref)} keeps the reference of its own vertex which is present in the \vl. \en{} points the next \enode{} of the \el{}.
}
%\vspace{-.3cm}
\begin{algorithm}
	\scriptsize 
	\caption{\cminer{(\aul, STM)}: Concurrently $m$ threads are executing atomic-units of smart contract from \aul{}(or list of atomic-units) with the help of STM.}
	\label{alg:cminer}	
	\begin{algorithmic}[1]
		\makeatletter\setcounter{ALG@line}{0}\makeatother
		\Procedure{\cminer{(\aul, STM)}}{}\label{lin:cminer1}
		\State curAU $\gets$ $curInd$.$get\&Inc(\aul)$; \label{lin:cminer2}
		\State /*curAU is the current atomic-unit taken from the \aul*/
		\State /*Execute until all the atomic-units successfully completed*/\label{lin:cminer3}
		\While{(curAU $<$ size\_of(\aul))}\label{lin:cminer4}
		\State $T_i$ $\gets$ STM.\begtrans{()};/*Create a new transaction $T_i$ with timestamp $i$*/\label{lin:cminer5}
		\While{(curAU.steps.hasNext())} /*Assume that curAU is a list of steps*/\label{lin:cminer6}
		\State curStep = currAU.steps.next(); /*Get the next step to execute*/\label{lin:cminer7}
		\Switch{(curStep)}\label{lin:cminer8}
		\EndSwitch
		\Case{read($x$):}\label{lin:cminer9}
		\State $v$ $\gets$ STM.\readi{($x$)}; /*Read \tobj{} $x$ from a shared memory*/\label{lin:cminer10}
		\If{($v$ == $abort$)}\label{lin:cminer11}
		\State goto \Lineref{cminer5};\label{lin:cminer12}
		\EndIf\label{lin:cminer13}
		\EndCase
		\Case{write($x, v$):} \label{lin:cminer14}
		\State /*Write \tobj{} $x$ into $T_i$ local memory with value $v$*/\label{lin:cminer15}
		\State STM.$write_i$($x, v$); \label{lin:cminer16}
		\EndCase
		\Case{default:}\label{lin:cminer17}
		\State /*Neither read from or write to a shared memory \tobj{}*/\label{lin:cminer18}
		\State execute curStep;\label{lin:cminer19}
		\EndCase
		\EndWhile\label{lin:cminer20}
		\State /*Try to commit the current transaction $T_i$ and update the \cl{[i]}*/\label{lin:cminer21}
		\State $v$ $\gets$ \tryc{$_i$()}; \label{lin:cminer22}
		\If{($v == abort$)}\label{lin:cminer23}
		\State goto \Lineref{cminer5};\label{lin:cminer24}
		\EndIf			\label{lin:cminer25}
		\State Create \vnode{} with $\langle$\emph{$i$, $AU_{id}$, 0, nil, nil}$\rangle$ as a vertex of Block Graph;	\label{lin:cminer26}
		\State BG(\emph{vNode}, STM);		\label{lin:cminer27}
		\State curAU $\gets$ $curInd$.$get\&Inc(\aul)$; \label{lin:cminer28}
		\EndWhile	\label{lin:cminer29}
		\EndProcedure\label{lin:cminer30}
		
	\end{algorithmic}
\end{algorithm}
%\vspace{-.3cm}

\tikz \node[circle,scale=.5,color=black, fill=pink]{\textbf{3}}; Once the transaction commits, it stores the conflicts in the block graph (or BG). To maintain the BG it calls addVert() and addEdge() methods of the lock-free graph library. The internal details of addVert() and addEdge() methods are explained in \subsecref{bg}. 
%In order to store the \emph{Conflict Graph} or \confg \emph{(CG(V, E))}, we are maintaining \emph{adjacency list}. In which all the vertices (or \vnode{s}) are stored in the vertex list (\vl{}) in increasing order of timestamp between the two sentinel node \vh{} (-$\infty$) and \vt{} (+$\infty$). Committed transaction $T_i$ creates the vertex node (or \vnode) as $\langle ts = i, AU_{id} = id, \inc{} = 0, \vn{} = nil, \en{} = nil\rangle$. Where $ts$ is a unique timestamp $i$ of committed transactions $T_i$ which is assigned at the beginning of it by STM.begin(). $AU_{id}$ is the $id$ of \au{} which is executed by transaction $T_i$. To maintain the indegree count of each \vnode{} we initialize \inc{} as 0. \vn{} and \en{} initializes as $nil$. At \Lineref{cg3}, it gets the list of conflicting transactions of $T_i$ with the help of STM.\emph{getConfList}(). Now, we maintain all the conflicts of \vnode{} in the edge list (\el) as shown in \figref{confg}. \el{} stores \enode{} (or conflicting transaction nodes say $T_j$) stores in increasing order of timestamp (or $ts$) between two sentinel nodes \eh{} (-$\infty$) and \et{} (+$\infty$). We maintain a conflict edge between the transaction $T_i$ and $T_j$ in \cgraph{} which is going from lower $ts$ to higher $ts$ to make the \cgraph{} acyclic at \Lineref{cg6}. Before adding an edge in the \cgraph{} it checks that both the transactions \vnode{s} should be present in the \vl{} at \Lineref{adde2} and \Lineref{adde3}. If \vnode{} is not part of \vl{} then it creates a node and add it to the \vl{} at \Lineref{addv5} with the help of atomic \emph{compare and swap} operation.    
%After successful addition of \vnode{s} corresponding to the transactions $T_i$ and $T_j$ in \vl{}, \cgraph{} maintains the conflict edge in \el{}. Lets assume $ts$ of $T_i$ is less then the $ts$ of $T_j$. So conflict edge should go from $T_i$ to $T_j$. Transaction $T_i$ creates a edge node (or \enode{}) as $\langle$\emph{ts = j, vref}, \en{} = $nil$ $\rangle$. Here, $ts$ is a unique timestamp $j$ of \emph{committed} transaction $T_j$ which had a conflict with $T_i$. \emph{Vertex node reference (or vref)} keeps the reference of its own vertex which is present in the \vl. \en{} initializes as $nil$. After successful addition of \enode{} in the \el{} of \vnode{}, transaction $T_i$ increment the \inc{} of \enode.$vref$ node which is present in the \vl{} at \Lineref{adde8} because $T_j$ is having an incoming edge from $T_i$.  
\tikz \node[circle,scale=.5,color=black, fill=pink]{\textbf{4}}; Once the transactions successfully executed the \au{s} and completed with the construction of BG then \conminer{} compute the hash of the previous block. Eventually, \tikz \node[circle,scale=.5,color=black, fill=pink]{\textbf{5}}; \conminer{} propose a block which consists of set of transactions, BG, final state of each shared \tobj{s}, hash of the previous block of the blockchain and \tikz \node[circle,scale=.5,color=black, fill=pink]{\textbf{6}}; send it to all other existing node in the \emph{distributed shared memory} to validate it as shown in \figref{cminer}. 
 %in created in the \el{} of \vnode{}. Finally, The structure of \enode{} is as $\langle$\emph{$ts_j$, vref}, \en{} $\rangle$. $ts_j$ is a unique timestamp $j$ of \emph{committed} transaction $T_j$ which had a conflict with $T_i$. \emph{Vertex node reference (or vref)} keeps the reference of its own vertex which is present in the \vl. \en{} points the next \enode{} of the \el{}.


%\begin{itemize}
%\item \cachel{}: It contains the node whose \inc{} is 0. 
%\end{itemize}





\subsection{Concurrent Validator}
\label{subsec:cvalidator}
Concurrent validator validates the block proposed by the concurrent miner. 
%If the validation is successful i.e. final state derived from \convalidator{} matches with the final state given by the \conminer{} and satisfies a consensus mechanism then proposed block is added into the \bc{} and \conminer{} who appended the block is rewarded. 
It executes the set of transactions concurrently and deterministically with the help of block graph given by the \conminer{}. BG consists of dependency among the conflicting transactions that restrict them to execute serially whereas non-conflicting transactions can run concurrently.
In \convalidator{} multiple threads are executing the \au{s} of \SContract{s} concurrently by \emph{executeCode()} method at \Lineref{sl4} and \Lineref{sl41} with the help of searchLocal(), and searchGlobal() and decInCount() methods of lock-free graph library at \Lineref{val5}, \Lineref{val16} and (\Lineref{val8}, \Lineref{val20}) respectively. %It gets the $AU_{id}$ from the searchLocal() and searchGlobal() and execute it by executeCode() method at \Lineref{sl4} and \Lineref{sl41}. 
The functionality of these lock-free graph library methods are explained in \subsecref{bg}. 
 %Multiple threads are going to execute the \convalidator{} function concurrently. 
% First, each validator thread  identifies the source node (having a indegree (or \inc) 0) in its local \cachel{} at \Lineref{cvalidator5}. To optimize the searching time of identifying the source node in \cgraph{}, each thread locally maintains the \cachel{} which consist of source node identified while executing the \au{} of corresponding to \vnode{}.

%If any source node exist in the local \cachel{} with \inc{} 0 then its \inc{} field is atomically sets to be -1 at \Lineref{searchl4}. After that validator thread executes the \au{s} corresponding to that source node concurrently at \Lineref{searchl7} and compute the other valid state. After successful execution of \au{} it decreases the \inc{} of all conflicting nodes atomically which is present in the \el{} corresponding to that source node at \Lineref{searchl9}. While decrementing the \inc{} of each conflicting nodes in the \cgraph{}, it again checks if any conflicting node became a source node then it adds that node into its local \cachel{} which optimize the search time of identifying the next source node from \cgraph. 

%Once all the source node executed from the local \cachel{}, \Validator{} threads identify the source node in the \cgraph{} at \Lineref{cvalidator6} and execute them same as above. Validator threads identify the source node in the \cgraph{} until all the \vnode's \inc{} became -1 i.e. all the \vnode{s} or \au{s} have been executed by the threads.

After the successful execution of all the \au{s}, \convalidator{} compares its computed final state of each shared data-objects with the final states given by the \conminer{}. If the final state matches for all the shared data-objects then the block proposed by the \conminer{} is valid. Finally, the block is appended to the blockchain and respective \conminer{} is rewarded.
%\vspace{-.3cm}
\begin{algorithm}
\scriptsize
	\caption{\cvalidator{(\aul, BG)}: Concurrently $V$ threads are executing atomic-units of smart contract with the help of BG given by the miner.}
	%	\textbf{Input:} m (\# miner threads); \textit{list AUs[]} (list of Atomic Units); conf\_graph (conflict graph generated by miner); Gnode\_count (\# node in graph).\\
	%	\textbf{Output:} Final state of Smart Contract.
	\begin{algorithmic}[1]
		%		\State atomic $eCounter$ = 0; 
		\makeatletter\setcounter{ALG@line}{31}\makeatother
		\Procedure{\cvalidator{(\aul, BG)}}{}		
		\State /*Execute until all the atomic-units successfully completed*/ \label{lin:val1}
		\While{(\nc{} $<$ size\_of(\aul))} \label{lin:val2}
		\While{(\cachel{}.hasNext())} /*First search into thread local \cachel*/\label{lin:val3}
		\State cacheVer $\gets$ \cachel{}.next(); \label{lin:val4}
		\State cacheVertex $\gets$ \searchl{(cacheVer, $AU_{id}$)};\label{lin:val5}
%		\State /*Execute the atomic unit of cacheVer (or cacheVer.$AU_{id}$)*/\label{lin:sl3}
		\State  \exec{($AU_{id}$)};\label{lin:sl4} /*Execute the atomic-unit of cacheVertex*/
%		\If{(cacheVertex)}\label{lin:val6}
		\While{(cacheVertex)}\label{lin:val7}
		\State cacheVertex $\gets$ decInCount(cacheVertex);\label{lin:val8}
	
%		\State cacheVertex $\gets$ cacheVertex.\en;\label{lin:val9}
		\EndWhile\label{lin:val10}
%		\EndIf\label{lin:val11}
		\State Remove the current node (or cacheVertex) from local \cachel; \label{lin:val12}
		\EndWhile\label{lin:val13}
%		\State verNode $\gets$ true;
%		\While{(verNode)}\label{lin:val15}%/*Search into the BG*/
		\State vexNode $\gets$ \searchg{(BG, $AU_{id}$)}; /*Search into the BG*/\label{lin:val16}
		\State  \exec{($AU_{id}$)};\label{lin:sl41} /*Execute the atomic-unit of vexNode*/		
%		\If{(verNode)}\label{lin:val17}
%		\State \enode $\gets$ vexNode.\eh;\label{lin:val18}
		\While{(verNode)}\label{lin:val19}
		\State verNode $\gets$ decInCount(verNode);\label{lin:val20}
		%\State \enode $\gets$ \enode.\en;\label{lin:val21}
		\EndWhile\label{lin:val22}
%		\EndIf\label{lin:val23}
%		\State \searchl();
		%\State \vnode $\gets$ \vnode.\vn;\label{lin:val24}
%		\EndWhile\label{lin:val25}
%		\State return$\langle void \rangle$;\label{lin:val26}
		\EndWhile\label{lin:val27}
		\EndProcedure
	\end{algorithmic}
\end{algorithm}
%\vspace{-.3cm}
\begin{theorem}
	All the dependencies between the conflicting nodes are captured in the BG.
\end{theorem} 

	





\cmnt{
\begin{algorithm}
	\scriptsize
	\label{alg:cvalidator} 	
	\caption{\cvalidator(): Concurrently $V$ threads are executing atomic units of smart contract with the help of $CG$ given by the miner.}
	%	\textbf{Input:} m (\# miner threads); \textit{list AUs[]} (list of Atomic Units); conf\_graph (conflict graph generated by miner); Gnode\_count (\# node in graph).\\
	%	\textbf{Output:} Final state of Smart Contract.
	\begin{algorithmic}[1]
		%		\State atomic $eCounter$ = 0; 
		\makeatletter\setcounter{ALG@line}{69}\makeatother
		\Procedure{\cvalidator()}{} \label{lin:cvalidator1}
		\State /*Execute until all the atomic units successfully completed*/\label{lin:cvalidator2}
		\While{(\nc{} $<$ size\_of(\aul))}\label{lin:cvalidator3}
		\State \vnode{} $\gets$ $CG$.\vh;\label{lin:cvalidator4}
		\State \searchl();/*First search into the thread local \cachel*/\label{lin:cvalidator5}
		\State \searchg(\vnode);/*Search into the \confg*/\label{lin:cvalidator6}
		%		\Procedure{{\color{blue}$concValidator(t\_ID)$}}{}
		%\State curGNode $\gets$ $curVInd$.$get\&Inc()$;
		%\State verTemp = conf\_grpah$\rightarrow$verHead$\rightarrow$Next;
		\EndWhile \label{lin:cvalidator7}
		\EndProcedure\label{lin:cvalidator8}
	\end{algorithmic}
\end{algorithm}


\begin{algorithm}
	\scriptsize
	\label{alg:searchl} 	
	\caption{\searchl(): First thread search into its local \cachel{}.}
	%	\textbf{Input:} m (\# miner threads); \textit{list AUs[]} (list of Atomic Units); conf\_graph (conflict graph generated by miner); Gnode\_count (\# node in graph).\\
	%	\textbf{Output:} Final state of Smart Contract.
	\begin{algorithmic}[1]
		%		\State atomic $eCounter$ = 0; 
		\makeatletter\setcounter{ALG@line}{77}\makeatother
		\Procedure{\searchl()}{}\label{lin:searchl1}
		\While{(\cachel{}.hasNext())}/*First search into the local nodes list*/\label{lin:searchl2}
		\State cacheVer $\gets$ \cachel{}.next(); \label{lin:searchl3} 
		%		\State \opt{(cacheVer)};
		\If{( cacheVer.\inc.CAS(0, -1))} \label{lin:searchl4}
		\State \nc{} $\gets$ \nc{}.$get\&Inc()$; \label{lin:searchl5}
		%		\State \nc{} $\gets$ \nc{} + 1;
		\State /*Execute the atomic unit of cacheVer (or cacheVer.$AU_{id}$)*/ \label{lin:searchl6}
		\State  \exec(cacheVer.$AU_{id}$);\label{lin:searchl7}
		\While{(cacheVer.\eh.\en $\neq$ cacheVer.\et)} \label{lin:searchl8}
		\State Decrement the \emph{inCnt} atomically of cacheVer.\emph{vref} in the \vl{}; \label{lin:searchl9} 
		\If{(cacheVer.\emph{vref}.\inc{} == 0)}\label{lin:searchl10}
		\State Update the \cachel{} of thread local log, \tl{}; \label{lin:searchl11}
		\EndIf\label{lin:searchl12}
		\State cacheVer $\gets$ cacheVer.\en;\label{lin:searchl13}
		\EndWhile\label{lin:searchl14}
		\Else\label{lin:searchl15}
		\State Remove the current node (or cacheVer) from the list of cached nodes; \label{lin:searchl16}
		\EndIf\label{lin:searchl17}
		
		\EndWhile\label{lin:searchl18}
		\State return $\langle void \rangle$;\label{lin:searchl19}
		\EndProcedure\label{lin:searchl20}
	\end{algorithmic}
\end{algorithm}


\begin{algorithm}
	\scriptsize
	\label{alg:searchg} 	
	\caption{\searchg(\vnode): Search the \vnode{} in the \confg{} whose \inc{} is 0.}
	%	\textbf{Input:} m (\# miner threads); \textit{list AUs[]} (list of Atomic Units); conf\_graph (conflict graph generated by miner); Gnode\_count (\# node in graph).\\
	%	\textbf{Output:} Final state of Smart Contract.
	\begin{algorithmic}[1]
		%		\State atomic $eCounter$ = 0; 
		\makeatletter\setcounter{ALG@line}{97}\makeatother
		\Procedure{\searchg(\vnode)}{} \label{lin:searchg1}
		\While{(\vnode.\vn{} $\neq$ $CG$.\vt)}/*Search into the \confg*/ \label{lin:searchg2}
		\If{( \vnode.\inc.CAS(0, -1))} \label{lin:searchg3}
		\State \nc{} $\gets$ \nc{}.$get\&Inc()$; \label{lin:searchg4}
		%		\State \nc{} $\gets$ \nc{} + 1;
		\State /*Execute the atomic unit of \vnode (or \vnode.$AU_{id}$)*/\label{lin:searchg5}
		\State  \exec(\vnode.$AU_{id}$);\label{lin:searchg6}
		%				\State  Execute the atomic unit of \vnode (or \vnode.$AU_{id}$).
		\State \enode $\gets$ \vnode.\eh;\label{lin:searchg7}
		\While{(\enode.\en{} $\neq$ \enode.\et)}\label{lin:searchg8}
		\State Decrement the \emph{inCnt} atomically of \enode.\emph{vref} in the \vl{};\label{lin:searchg9} 
		\If{(\enode.\emph{vref}.\inc{} == 0)}\label{lin:searchg10}
		\State /*\cachel{} contains the list of node which \inc{} is 0*/\label{lin:searchg11}
		\State Add \enode.\emph{verf} node into \cachel{} of thread local log, \tl{}; \label{lin:searchg12}
		\EndIf \label{lin:searchg13}
		\State \enode $\gets$ \enode.\en; \label{lin:searchg14}
		\EndWhile\label{lin:searchg15}
		\State \searchl();\label{lin:searchg16}
		\Else\label{lin:searchg17}
		\State \vnode $\gets$ \vnode.\vn;\label{lin:searchg18}
		\EndIf\label{lin:searchg19}
		\EndWhile\label{lin:searchg20}
		\State return $\langle void \rangle$;\label{lin:searchg21}
		\EndProcedure\label{lin:searchg22}
	\end{algorithmic}
\end{algorithm}
}




==> Arxiv version Archit pdp-19-bc (H space) (copy)/results.tex <==

\cmnt{
\section{IMPLEMENTATION}
%For the experiment, we have chosen smart contracts from Solidity documentation [].
In Ethereum blockchain, smart contracts are written in Turing complete language Solidity and runs on the Ethereum Virtual Machine (EVM). The issue with EVM is that it does not support multi-threading and hence give poor throughput. Therefore, to exploit the efficient utilization of multi-core resources and to improve the performance, we have converted smart contract from Solidity language into C++ and executed them using multi-threading. %\todo{We r not modifying the contract. It has to rewrite. \\RESOLVED}\todo{What I mean by modifying is, that converted C++ contract is modified/ now, I changed it to instrumented} 
Further, contracts are instrumented to use STM library [], the methods of the contracts are converted into an atomic section know as Atomic Units (AUs).% The struct type of the Solidity contract is converted into the C++ structure, and mapping is implemented as a hash map.


%For the experiment, we have chosen smart contracts from Solidity documentation [3]. These contracts are written in contract-oriented, high-level language Solidity and runs on the Ethereum Virtual Machine (EVM), but the issue with EVM is that it does not support multi-threading and hence give poor throughput. Therefore, to exploit the efficient utilization of multi-core resources and to improve the performance, we have converted smart contracts in C++ and executed them using multi-threading. In this process, contract methods are modified to use STM library []. Each method of the contract is converted into an atomic section know as Atomic Units (AUs), and shared data of the contract is instrumented to use STM shared memory. The struct type of Solidity is replaced with C++ structure. Mapping data types are implemented as a concurrent hash map. The STM system provides all the basic needs of concurrent execution.

\todo{If you thing this pera is not important then we can remove this, but reviewer may ask what is difference between fork-join and decentralized approach.}The miners execute the AUs concurrently using multiple threads and record the dependencies in the \textit{block graph}. After successful execution of an AU, the same thread adds the respective node and edges in the \textit{block graph} by using methods of the concurrent graph library. A graph node includes all the required details about the AUs. Edges in the graph are added based on the increasing order of the time stamps which ensures that there will be no cycle hence no deadlock. Further, during concurrent execution of the AUs, if any AU is aborted, it is re-executed by the same thread until it succeeds. Later, validator uses the \textit{block graph} to re-executes the atomic units based on two approaches \textit{fork-join} and \textit{decentralized}. In the \textit{fork-join} approach, a master thread creates a pool of worker threads and assigns them AUs based on the \textit{indegree} of the graph nodes. While in the \textit{decentralized approach}, thread themselves identify the node/AU's having \textit{indegree} zero to execute in the graph, claims the ownership of the node, and then finally execute. Finally, thread changes the \textit{indegree} of all the nodes having an incident edge from the current node.%\todo{\scriptsize We can move this paragraph in proposed mechanism. Yes, we can, only thing is concurrent validator is different the way they implemented. So its better to explain generalized validator in proposed mechanism, and here this paragraph will give some insights.}
}

\section{EXPERIMENTAL EVALUATION}
%Our objective is to increase throughput by allowing concurrent execution of contracts by miners and validators. 
For the experiment, we consider a set of benchmarks generated for Ballot, Simple Auction, and Coin contracts from Solidity documentation \cite{Solidity}. Experiments are performed by varying the number of atomic-units, and threads. The analysis focuses on two main objectives: (1) Evaluate and analyzes the speedup achieved by concurrent miner over the serial miner. (2) Appraise the speedup achieved by concurrent validator over serial validator on various experiments.% We expect concurrent miner and validator to perform better than serial miner and validator.% However, when there is a high contention due to conflicting accesses to shared data objects drop in speedup can also be seen.

%Our objective is to increase throughput by allowing concurrent execution of contracts by miners and validators. For the evaluation of the proposed approach, we consider three contracts from solidity documentation and a set of benchmarks are generated for Ballot, Simple Auction, and Coin contracts. Benchmark results are analyzed by varying the number of threads, atomic units, and shared data objects. The experiments are carried out with two main objectives: the first is to evaluate the speedup achieved by concurrent miner over the serial miner and second to assess the speedup achieved by concurrent validator over serial validator. We expect concurrent miner and validator to perform better than serial miner and validator. %However, when there is a high contention due to conflicting accesses to shared data objects drop in speedup can also be seen.
\noindent \textbf{Experimental system:} The Experimental system is a large-scale 2-socket Intel(R) Xeon(R) CPU E5-2690 v4 @ 2.60 GHz with 14 cores per socket and two hyper-threads (HTs) per core, for a total of 56 threads. The machine has 32GB of RAM and runs Ubuntu 16.04.2 LTS.


%\noindent \textbf{STM implementations:}  We take the implementation of an efficient framework as BTO STM \cite[Chap 4]{WeiVoss:TIS:2002:Morg} and MVTO STM \cite{Kumar+:MVTO:ICDCN:2014} to execute the smart contracts concurrently.

\noindent \textbf{Methodology:} We have considered two types of workload, (W1) The number of atomic-units varies from 50 to 400, while threads and shared data-objects are fixed to 50 and 40 respectively. (W2) The number of threads varies from 10 to 60 while atomic-units are fixed to 400 and shared data-objects to 40. In all the experiments time taken by miners and validators is collected as an average of ten executions for the final result. 
\vspace{-.5cm}
%\noindent
\subsection{Benchmarks}
%We consider three benchmarks, Ballot, Simple Auction and Coin contracts. However, 
In reality, miner forms a block which consists of a set of transactions from different contracts. So, we consider four benchmarks Ballot, Simple Auction, Coin including Mixed contract which is the combination of above three. In Ethereum blockchain, smart contracts are written in Solidity and runs on the Ethereum Virtual Machine (EVM). The issue with EVM is that it does not support multi-threading and hence give poor throughput. Therefore, to exploit the efficient utilization of multi-core resources and to improve the performance, we convert smart contract from Solidity language into C++ and execute them using multi-threading. %\todo{We r not modifying the contract. It has to rewrite. \\RESOLVED}\todo{What I mean by modifying is, that converted C++ contract is modified/ now, I changed it to instrumented} 
%Further, contracts are instrumented to use STM library to make the methods of the contracts are converted into an atomic section know as Atomic Units (AUs).% which consists of contract transactions from Ballot, Simple Auction, and Coin contract. Other than Mixed all other benchmarks are conventional, by conventional we mean that entire block formation operates on the transactions from the same contract. 
The details of the benchmarks are as follows:
\begin{enumerate}
    \item \textbf{Simple Auction:} It is an auction contract in which \textit{bidders, highest bidder}, and \textit{highest bid} are the shared data-objects. A single owner initiates the auction after that bidders can bid in the auction. The termination condition for auction is the bidding period (or end time) initialized at the beginning of the auction. During bidding period multiple bidders initiate their bids with biding amount using \textit{bid()} method. At the end of the auction, a bidder with the highest amount will be successful, and respective bid amount is transferred to the beneficiary account. %Bid amount of all other failed bidders is kept in pending returns and transferred to corresponding address/bidder wallet. For benchmark, the state of the contract changes whenever a new bid with a higher amount succeeds. All the AUs of the block are requested to bidPlusOne() or withdraw(). The current bidder can request for bidPlusOne(). Whenever current bidder amount of bid is higher than the previous highest bid than in the first step current highest bid amount is transfers to the previous highest bidder pending account. Later in second step highest bid and bidder is updated. 
    Conflict can occur if at least two bidders are going to request for bidPlusOne() simultaneously. %Such conflicts can very much transpire when \emph{miner} executes contract concurrently.% Such conflicts can very much transpire when \emph{miner} executes contracts concurrently. We are dealing with these conflicts with the help of optimistic STMs and ensuring consistency.
   
    \item \textbf{Coin:} It is the simplest form of a cryptocurrency in which accounts are the shared data-objects. All accounts are uniquely identified by Etherum addresses. Only the contract deployer known as minter will be able to generate the coins and initialize the accounts at the beginning. Anyone having an account can send coins to another account with the condition that they have sufficient coins in their account or can check their balance. In the initial state, minter initializes all the accounts with some coins. %All the AUs of the block are requested to send() or getbalance().
    Conflict can occur if at least two senders are transferring the amount into the same receiver account simultaneously or when one send() and getbalance() have an account in common.% Such conflicts can very much transpire when \emph{miner} executes contracts concurrently. Optimistic STMs is used to ensuring consistency and to handle this conflicts.
    \item \textbf{Ballot: }% The basic idea behind Ballot contract is to create one contract per ballot. 
It implements an electronic voting contract in which voters and proposals are the shared data-objects. All the voters and proposals are already registered and have unique Ethereum address. At first, all the voters are given rights by the chairperson (or contract deployer) to participate in the ballot. Voters either cast their vote to the proposal of their choice or delegate vote to another voter whom they can trust using delegate(). A voter is allowed to delegate or vote once throughout the ballot. Conflict can occur if at least two voters are going to delegate their vote to the same voter or cast a vote to the same proposal simultaneously.  %We are handling this conflicts with the help of optimistic STMs and ensuring consistency. 
Once the ballot period is over, the winner of the ballot is decided based on the maximum vote count.% Vote counting is done atomically and transparently.  
    \item \textbf{Mixed:} In this benchmark, we have combined all the above benchmarks in equal proportions. Data conflicts occur when AUs of the same contract executed simultaneously, and operate on common shared data-objects. 
\end{enumerate}
In all the above contracts, conflicts can very much transpire when \emph{miner} executes them concurrently. So, we use Optimistic STMs to ensure consistency and handle the conflicts. 
 \vspace{-.2cm}
%\noindent
\subsection{Results}

%\textit{B. Results}\\
%For each benchmark execution, blocks were created by including the number of AUs depending on the workloads. AUs in each block is executed by a concurrent miner, a concurrent validator, a serial miner, and a serial validator. 
\noindent
%Experiments are performed multiple time for workload W1 and W2 to identify the best parameters. 
We have shown the speedup of concurrent execution by miner and validator over serial in Table I. The results from the serial execution of the miner and validator are served as the baseline. %A series of experiments have been performed to reach till conclusion. The execution time is averaged over ten runs. 

%\vspace{-.6cm}
 \begin{figure}
 	\centering
 	%      	\captionsetup{justification=centering}
 	{\includegraphics[width=9cm]{figs/simplecoin.pdf}}
 	% \vspace{-16cm}
\vspace{-.8cm} 	\caption{Simple Auction and Coin Contracts}
 	\label{fig:asc}
 \end{figure}
%\vspace{-.45cm}
\figref{asc} and \figref{bmc} represent the speedup of concurrent miner and validator relative to the serial miner and validator for all the smart contracts on workload W1 and W2. It shows average speedup of 3.6x and 3.7x by the BTO and MVTO concurrent miner over serial miner respectively. Along with, BTO and MVTO validator outperforms average 40.8x and 47.1x than serial validator respectively \footnote{Code is available here: https://github.com/pdcrl/Blockchain}. The maximum speedup by concurrent miner on workload W1 is achieved at the smaller number of atomic-units. On workload W2 speedup of concurrent miner increases while increasing the number of threads up to fix number depending on system configuration.

The time taken by the concurrent validator is negligible as compared to serial validator because concurrent validator executes contracts concurrently and deterministically using BG given by concurrent miner. BG simplifies the parallelization task for the validator as validator need not to determine the conflicts, and directly executes non-conflicting transactions concurrently. %A fork-join approach from Dickerson et al. [] also implemented for the concurrent validators using block graph given by concurrent miner through BTO STM and MVTO STM.
It is clear from \figref{asc} and \figref{bmc} that BTO and MVTO Decentralized Validator is giving far better performance than BTO and MVTO Fork-join Validator. A possible reason can be master thread of BTO and MVTO Fork-join Validator becomes slow to assign the task to slave threads. 
\cmnt{
\begin{table*}[ht] \centering
	\begin{tabular}{|c|l|l|l|}
		\hline
		\multicolumn{1}{|c|}{Simple Auction} & \multicolumn{1}{c|}{Coin} & \multicolumn{1}{c|}{Ballot} & \multicolumn{1}{c|}{Mixed}\\
		%S. No. & Sequence & Action \\
		\hline
		&  &  &\\
		\hline
		&  &  &\\
		\hline
		&  &  &\\
		\hline
		&  &  &\\
		\hline
		&  &  &\\
		\hline
		&  &  &\\
		%T50 cannot create the version and, hence, must be aborted\\
		\hline
	\end{tabular}
	\caption{Average speedups for each benchmark}
	\label{tbl:speedup}
\end{table*}
}
 %As shown in Figure 4 (a), The maximum speedup for concurrent miner using BTO STM and MVTO STM is achieved at 100 atomic-units while best speedup for concurrent validator is produced at 350 atomic-units.
%\vspace{-.5cm}
\begin{table}
	\caption{Speedup achieved by concurrent Miner and Validator}
	\vspace{-.3cm}
	\label{tbl:speedup}
	\resizebox{.49\textwidth}{!}{%
		\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
			\hline
			\multirow{2}{*}{} & \multicolumn{2}{c|}{\textbf{Simple Auction}} & \multicolumn{2}{c|}{\textbf{Coin}} & \multicolumn{2}{c|}{\textbf{Ballot}} & \multicolumn{2}{c|}{\textbf{Mixed}} \\ \cline{2-9} 
			& \textbf{W1} & \textbf{W2} & \textbf{W1} & \textbf{W2} & \textbf{W1} & \textbf{W2} & \textbf{W1} & \textbf{W2} \\ \hline
			\textbf{BTO Miner} & 4.6 & 2.4 & 6.6 & 2.1 & 3.8 & 3.1 & 4.8 & 1.6 \\ \hline
			\textbf{MVTO Miner} & 5.2 & 2.7 & 7.5 & 2.4 & 2.3 & 1.5 & 5.7 & 1.8 \\ \hline
			\textbf{BTO Decentralized Validator} & 85.7 & 53.1 & 36.9 & 21.7 & 126.7 & 152.1 & 90.7 & 68.6 \\ \hline
			\textbf{MVTO Decentralized Validator} & 108.5 & 64.6 & 43.5 & 24.4 & 135.8 & 180.8 & 109.5 & 67.4 \\ \hline
			\textbf{BTO Fork-join Validator} & 1.7 & 2.5 & 1.7 & 2.1 & 2.1 & 3.8 & 1.5 & 1.9 \\ \hline
			\textbf{MVTO Fork-join Validator} & 1.5 & 2.3 & 1.9 & 2.3 & 1.8 & 3.8 & 1.5 & 2.7 \\ \hline
		\end{tabular}%
	}
\end{table}
%\vspace{-.4cm}
\figref{asc} shows the speedup achieved by concurrent MVTO  Miner is greater than BTO Miner for Simple Auction and Coin contract on workload W1 and W2 respectively. A plausible reason can be that MVTO gives good performance for read-intensive workloads \cite{Kumar+:MVTO:ICDCN:2014}. Here, Simple Auction and Coin contracts are read-intensive \cite{Solidity}. %200 AUs onwards, BTO Fork-join Validator outperforms MVTO Fork-join Validator because sometimes maintaining multiple versions leads to increase the search time for appropriate version.
 \figref{asc} (c) represents the speedup achieved by BTO and MVTO Fork-join Validators are even less than serial for 50 AUs due to the overhead of allocating the task by master thread. 
%\vspace{-.6cm}
\begin{figure}
	\centering
	%      	\captionsetup{justification=centering}
	{\includegraphics[width=9cm]{figs/ballotmixed.pdf}}
	% \vspace{-16cm}
\vspace{-.7cm}	\caption{Ballot and Mixed Contracts}
	\label{fig:bmc}
\end{figure}
%\vspace{-.45cm}

\figref{bmc} (a) and (b) capture better speedup achieved by concurrent BTO  Miner as compare to concurrent MVTO Miner for workload W1 and W2 because Ballot contract is write-intensive \cite{Solidity}. \figref{bmc} (c) and (d) represent the speedup achieved by concurrent miner and validator over serial miner and validator for the Mixed contract on workload W1 and W2 respectively. Due to equal proportions of all the above three contracts, the Mixed contract becomes read-intensive. So, the properties of the Mixed contract are same as Simple Auction and Coin contract with similar reasoning. Due to space constraints, we present essential results in the main paper and the remaining results on different workloads %like varying the shared data-objects, and average time taken by each contracts 
are available in the \apnref{rresult}.  


\cmnt{ 

In Figure 4 (a), it can be seen that with the increase in the number of AUs the speedup achieved by concurrent BTO  miner dominates the MVTO miner. A plausible reason can be that MVTO gives good performance for read-intensive workloads, however, for Ballot contract workload is write intensive. In Figure 4 (b, c), with the increase in the number of threads and shared objects respectively performance of MVTO and BTO miner increases gradually, however, for these workloads again, MVTO is not performing better then BTO and reason can be the same. 
%In all the workloads it is difficult to conclude that which decentralized validator (BTO  or MVTO) is giving better speedup than other, however decentralized validators are doing better then fork-join validators \todo{Wrong observation}. 
Further, fork-join is not performing better than decentralized validator a reason can be that master thread becomes slow to assign the task to slave threads.


%A possible reason for degradation in MVTO performance can be the increase in the number of versions of each shared data object with the increase in the number of AUs.

%Figure 4 represents the speedup of a concurrent miner and concurrent validator relative to the serial miner and validator for ballot contract on workloads W1, W2, and W3 respectively. The maximum speedup for concurrent miner using BTO STM and MVTO STM is achived at 100 atomic-units while best speedup for concurrent validator is achieved at 350 atomic-units, as shown in Figure 4 (a). The time taken by the concurrent validator is negligible as compared to serial because concurrent validators execute contracts concurrently and deterministically using block graph given by the concurrent miner. The block graph simplifies the parallelization task for the validator as validator need not to determine the conflicts, and directly executes non-conflicting transactions concurrently. A fork-join approach from Dickerson et al. [] is also implemented for the concurrent validators using block graph given by concurrent miner through BTO STM and MVTO STM \todo{Needs to modify and update the correct observations from graph}. 


%From Figure 4 it can be easily seen that for less number of atomic-units concurrent validators using fork-join is not performing better than serial this may be because the master thread becomes slow to assign the task to slave threads. Figure 4 (b) shows higher the number of threads better the speedup for the concurrent miner and concurrent validator because of higher system configuration. A notable observation here is that MVTO STM beats BTO STM and serial on high contention (with less number of shared data-objects) as represented in Figure 4 (c) \todo{Wrong observation}. A plausible reason behind this can be higher conflicts percentage which leads to more number of aborts in BTO STM  whereas MVTO STM maintains multiple versions, therefore, fewer number aborts \todo{Wrong observation}.

Figure 5, 6 represents the speedup achieved by concurrent miner and validator over serial for Simple Auction and Coin contracts. In both the contracts for workload W1 and W2 MVTO miner is giving better speedup over other miners as  workload is read-intensive. However, in Figure 5 (c), with the increase in the number of the shared data objects, after 40 shared objects, BTO miner start outperforming then MVTO miner because of the increase in search time for MVTO miner. For all three workloads in all the benchmarks, MVTO decentralized validator is performing better than others. A important observation here is that even fork-join validator is also doing better than serial in all workloads; this is because in the simple auction the workload is read-intensive therefore fewer conflicts/dependencies between AUs, hence more concurrency. % For W3, increment in the speedup for concurrent miner can be observed up to 40 shared objects after that it degrades. Because of the increase in search time.
Similarly, Figure 7 represents the speedup achieved for the Mixed benchmark. For all workloads, concurrent MVTO miner is doing better than BTO and serial miner. For mixed benchmark we have given equal weightage to all the contract AUs, and since Simple Auction and Coin is read-intensive, so overall workload is read-intensive. Further, for all workloads for almost all points, MVTO decentralized validator is better over all other validators. A reason can be read-intensive workload. 
}
%Finally, we can conclude that MVTO miner is giving better performance for read-intensive workloads and BTO miner is giving better speedup for write-intensive workloads, however, both concurrent miner producing better speedup over serial miner. Fork-join validator is doing better than serial but dominated by the decentralized validator.% On an average speedup achieved by the concurrent miner is XXX, decentralized validator is YYY, and fork-join validator is ZZZ.



